Semantic Logical Relations for Timed Message-Passing Protocols (Extended Version)

Many of today's message-passing systems not only require messages to be exchanged in a certain order but also to happen at a certain \emph{time} or within a certain \emph{time window}. Such correctness conditions are particularly prominent in Internet of Things (IoT) and real-time systems applications, which interface with hardware devices that come with inherent timing constraints. Verifying compliance of such systems with the intended \emph{timed protocol} is challenged by their \emph{heterogeneity} -- ruling out any verification method that relies on the system to be implemented in one common language, let alone in a high-level and typed programming language. To address this challenge, this paper contributes a \emph{logical relation} to verify that its inhabitants (the applications and hardware devices to be proved correct) comply with the given timed protocol. To cater to the systems' heterogeneity, the logical relation is entirely \emph{semantic}, lifting the requirement that its inhabitants are syntactically well-typed. A semantic approach enables two modes of use of the logical relation for program verification: (i) \emph{once-and-for-all} verification of an \emph{arbitrary} well-typed application, given a type system, and (ii) \emph{per-instance} verification of a specific application / hardware device (a.k.a. foreign code). To facilitate mode (i), the paper develops a refinement type system for expressing timed message-passing protocols and proves that any well-typed program inhabits the logical relation (fundamental theorem). A type checker for the refinement type system has been implemented in Rust, using an SMT solver to check satisfiability of timing constraints. Then, the paper demonstrates both modes of use based on a small case study of a smart home system for monitoring air quality, consisting of a controller application and various environment sensors.

==> apx/retyping.tex <==
Rules \ruleref{rule:fwd} and \ruleref{rule:cut} deserve special attention
because they require checking for \emph{temporal validity}.
The process $\tpfwdcst{T}{x}$ 
forwards all message from (and to) $x$ to (and from) its own providing channel. 
The process $\tpspawnproccst{T}{P}{x}{Q}$ spawns $P$ 
of type $A$ at time $T$ as a new process then communicates with it through $\IsOf{x}{A}$ 
by continuing with $Q$. The process $P$ provides $A$ and $Q$ becomes its client. 

For temporal \emph{soundness}, we must ensure that a forward does not happen ``too late'',
\ie that the process providing along $x$ must be available at least for the entire period that
the forwarding process promises to be available to its client.
Rule \ruleref{rule:fwd} thus includes the premise
$\calG; \calF \entails{\FwdComp{A}{A'}{T}}$.
This judgment asserts that $A$ can be safely forwarded as $A'$ at time $T$.
To see what goes wrong otherwise, 
consider the following process:
$$
\begin{small}
p(t) \triangleq \fbetween{t_0}{t}{\fshiftcst{t_0}{5}} \qquad 
t_0;\, \calF \mid 
\IsOf{x}{\tpunitstycst{t}{p(t)}}, 
\IsOf{y}{\tpunitstycst{t}{p(t)}} 
\entails{\IsOfProc{\tpwaitcst{\fshiftcst{t_0}{2}}{y}{\tpfwdcst{\fshiftcst{t_0}{2}}{x}}}{t}{\tpunitstycst{t}{p(t)}}}
\end{small}
$$
The process starts at $t_0$ and waits until $\fshiftcst{t_0}{2}$ to close $y$, then 
it starts forwarding $x$. Itself, it advertises to be available $\fbetween{t_0}{t}{\fshiftcst{t_0}{5}}$ along its providing channel,
which includes $\fshiftcst{t_0}{1}$.
At this time, however, it will not be available as it communicates with $y$.
This is a soundness problem pertaining specifically to \ruleref{rule:fwd}. 

A dual problem of \emph{completeness} arises in the \ruleref{rule:cut}~rule. 
Suppose at time $\fshiftcst{t_0}{2}$ we 
have a provider $P$ and client $Q$ satisfying: 

\begin{small}
$$\Delta_1 \entails{\IsOfProc{P}{\fshiftcst{t_0}{2}}{\tpunitstycst{t}{\leqcst{\fshiftcst{t_0}{2}}{t}}}},
\quad 
\Delta_2, \IsOf{x}{\tpunitstycst{t}{t_0 \leq t}} 
\entails{\IsOfProc{Q}{\fshiftcst{t_0}{2}}{C}}$$
\end{small}
Process $Q$ expects to be able to close $x$ at any time following $t_0$, and $P$ is a process 
that can be closed at any time after $\fshiftcst{t_0}{2}$. However, since the typing is 
derived at $\fshiftcst{t_0}{2}$, the earliest possible time that $Q$ can communicate through 
$x$ is the current time $\fshiftcst{t_0}{2}$.
Therefore, this cut should be permitted, despite the fact that the types provided and used are syntactically different.
To facilitate such cuts, rule \ruleref{rule:cut} includes the premise $\calG; \calF \entails{\CutComp{A}{A'}{T}}$,
termed \emph{cut retyping}. The judgment asserts 
$A$ can be used as $A'$ in a context at $T$.
%
We omit definition of the both retyping judgments due to space limitations, 
The definitions are included in \cref{apx:lang:statics:retyping}.

==> apx/sem-tlogic.tex <==
\begin{definition}[Interpretation]
Fix a temporal structure $\calM$, we \emph{interpretations} for elements of sorts 
$\Sort{Time}$, $\Sort{Duration}$ mutual inductively as follows:
\begin{align*}
\Interp{T} &: (\FV{T} \to \bbT) \to \bbT \\
\Interp{D} &: (\FV{D} \to \bbT) \to \bbD \\
\\
\InterpA{t}{\varphi} &\triangleq \varphi(t) \\
\InterpA{\fshiftcst{T}{D}}{\varphi} &\triangleq \InterpA{T}{\varphi} + \InterpA{D}{\varphi} \\
\InterpA{\finitcst}{\varphi} &\triangleq i \\
\\
\InterpA{\dzerocst}{\varphi} &\triangleq z \\
\InterpA{\dunitcst}{\varphi} &\triangleq u \\
\InterpA{\dsumcst{D_1}{D_2}}{\varphi}  &\triangleq \InterpA{D_1}{\varphi} \oplus \InterpA{D_2}{\varphi} \\ 
\InterpA{\ddiffcst{T_1}{T_2}}{\varphi} &\triangleq \InterpA{T_1}{\varphi} - \InterpA{T_2}{\varphi} \\
\end{align*}
\end{definition}

\begin{definition}[Interpretation, Cont.]
The interpretation is extended $\Sort{Prop}$ as follows:  
\begin{align*}
\Interp{P} &: (\FV{T} \to \bbT) \to \kw{prop} \\
\\
\InterpA{\topcst}{\varphi} &\triangleq \top \\
\InterpA{\botcst}{\varphi} &\triangleq \bot \\
\InterpA{\landcst{p_1}{p_2}}{\varphi} &\triangleq \InterpA{p_1}{\varphi} \land \InterpA{p_2}{\varphi} \\
\InterpA{\lorcst{p_1}{p_2}}{\varphi} &\triangleq \InterpA{p_1}{\varphi} \lor \InterpA{p_2}{\varphi} \\
\InterpA{\limpcst{p_1}{p_2}}{\varphi} &\triangleq \InterpA{p_1}{\varphi} \supset \InterpA{p_2}{\varphi} \\
\InterpA{\leqcst{T_1}{T_2}}{\varphi} &\triangleq \InterpA{T_1}{\varphi} \leq \InterpA{T_2}{\varphi} \\
\\
\end{align*}
\end{definition}

\begin{lemma}[Canonicity] Closed $T$ and $D$ has a canonical form.
\begin{itemize}
\item If $\emptyset; \calF \entails{\IsTime{T}}$ then $\emptyset; \emptyset \entails{\eqcst{T}{\fshiftcst{\finitcst}{\overline{n}}}}$ for some $\overline{n}$.
\item If $\emptyset; \calF \entails{\IsDuration{D}}$ then $\emptyset; \emptyset \entails{\eqcst{D}{\overline{n}}}$ for some $\overline{n}$.
\end{itemize}	
\end{lemma}
\begin{proof}
We will need to prove both by induction over the well-formedness judgment simultaneously. Most cases are exercises of using 
commutativity and associativity on durations. The critical case is to handle differences in time. Consider $\ddiffcst{T_1}{T_2}$, 
since both $T_1$ and $T_2$ by induction have canonical forms $\fshiftcst{\finitcst}{\overline{n_1}}$
and $\fshiftcst{\finitcst}{\overline{n_2}}$. The difference is then $\overline{n_1 - n_2}$.
\end{proof}

\begin{corollary}
For closed elements of time $T_1$ and $T_2$, the axiom of tricotomy is admissible.
\end{corollary}
\begin{proof}
Consider their canonical form and construct proof of ordering by examining the duration attached.
\end{proof}

\begin{corollary}\label{apx:cor:tri}
For closed elements of time $T_1$ and $T_2$, exactly one of the following is admissible without assumptions: 
$T_1 < T_2$, $T_1 = T_2$, or $T_1 < T_2$.
\end{corollary}
\begin{proof}
Because tricotomy is admissible, suffices to show no two can be true at the same time. If any pair of them 
are true at the same time, then the logic is inconsistent. Our logic has a nontrivial model, therefore it is 
consistent. The proof allows us to case split formal ordering between any pair of closed elements in time.
\end{proof}

\begin{corollary}
For closed elements of time $T_1$ and $T_2$, if $\Interp{T_1} \leq \Interp{T_2}$ then we can prove $T_1 \leq T_2$.
\end{corollary}
\begin{proof}
By \cref{apx:cor:tri}, either $T_1 \leq T_2$ or $T_1 > T_2$. If $T_1 > T_2$ then $\Interp{T_1} > \Interp{T_2}$, 
contradiction.
\end{proof}

As a consequence, we can define $\max(T_1, T_2)$ and $\min(T_1, T_2)$ for closed elements of $T_1$ and $T_2$. 


==> contents/lr.tex <==
\clearpage 
\section{Semantic Soundness}
\subsection{Temporal Structures}

% \begin{definition}
% A \emph{temporal structure} $\calM$ is a ten-tuple $\langle T, i, D, +, -, u, z, \oplus, \leq \rangle$, where 
% \begin{itemize}
%   \item $\bbT$ is the set of points in time.
%   \item $\bbD$ is the set of durations.
%   \item $i \in \bbT$ is the initial time.
%   \item $+ : \bbT \times \bbD \to \bbT$ \emph{shifts} its first argument by its second.
%   \item $- : \bbT \times \bbT \to \bbD$ computes the difference of two points in time for a duration.
%   \item $u \in \bbD$ is the unit duration; $z \in \bbD$ is the zero duration; 
%   \item $\oplus : \bbD \times \bbD \to \bbD$ sums durations.
%   \item $(\leq) : \bbT \times \bbT \to \kw{prop}$ a binary relation.
% \end{itemize}
% \end{definition}

% \begin{definition}[Assignment]
% Fix a temporal structure $\calM$, A \emph{(temporal) variable assignment of $\calG$}, 
% or just an \emph{assignment}, denoted by $\varphi$, is a function $\calG \to \bbT$.
% \end{definition}

% \begin{definition}[Interpretation]
% Fix a temporal structure $\calM$, we \emph{interpretations} for elements of sorts 
% $\Sort{Time}$, $\Sort{Duration}$ mutual inductively as follows:
% \begin{align*}
% \Interp{T} &: (\FV{T} \to \bbT) \to \bbT \\
% \Interp{D} &: (\FV{D} \to \bbT) \to \bbD \\
% \\
% \InterpA{t}{\varphi} &\triangleq \varphi(t) \\
% \InterpA{\fshiftcst{T}{D}}{\varphi} &\triangleq \InterpA{T}{\varphi} + \InterpA{D}{\varphi} \\
% \InterpA{\finitcst}{\varphi} &\triangleq i \\
% \\
% \InterpA{\dzerocst}{\varphi} &\triangleq z \\
% \InterpA{\dunitcst}{\varphi} &\triangleq u \\
% \InterpA{\dsumcst{D_1}{D_2}}{\varphi}  &\triangleq \InterpA{D_1}{\varphi} \oplus \InterpA{D_2}{\varphi} \\ 
% \InterpA{\ddiffcst{T_1}{T_2}}{\varphi} &\triangleq \InterpA{T_1}{\varphi} - \InterpA{T_2}{\varphi} \\
% \end{align*}
% \end{definition}

% \begin{definition}[Interpretation, Cont.]
% The interpretation is extended $\Sort{Prop}$ as follows:  
% \begin{align*}
% \Interp{P} &: (\FV{T} \to \bbT) \to \kw{prop} \\
% \\
% \InterpA{\topcst}{\varphi} &\triangleq \top \\
% \InterpA{\botcst}{\varphi} &\triangleq \bot \\
% \InterpA{\landcst{p_1}{p_2}}{\varphi} &\triangleq \InterpA{p_1}{\varphi} \land \InterpA{p_2}{\varphi} \\
% \InterpA{\lorcst{p_1}{p_2}}{\varphi} &\triangleq \InterpA{p_1}{\varphi} \lor \InterpA{p_2}{\varphi} \\
% \InterpA{\limpcst{p_1}{p_2}}{\varphi} &\triangleq \InterpA{p_1}{\varphi} \supset \InterpA{p_2}{\varphi} \\
% \InterpA{\leqcst{T_1}{T_2}}{\varphi} &\triangleq \InterpA{T_1}{\varphi} \leq \InterpA{T_2}{\varphi} \\
% \\
% \end{align*}
% \end{definition}

% \begin{definition}
% Given $\calG \entails{\IsProp{p}}$, an assignment is said to \emph{satisfy} 
% $p$, denoted $\Satisfy{\varphi}{p}$, iff $\InterpA{p}{\varphi}$. 
% An assignment satisfies a context $\calG \entails{\IsCtx{\calF}}$ iff for all 
% $p \in \calF$, $\Satisfy{\varphi}{p}$.
% \end{definition}

% \begin{notation}
% In contexts where the assignment $\varphi$ is clear, write $\Interp{-}$ for $\InterpA{-}{\varphi}$.
% \end{notation}

% \begin{definition}[Model]
% A temporal structure is a \emph{model} iff 
% for all $\calG; \calF \entails{p}$ and assignments $\varphi$ of $\calG$, 
% $\Satisfy{\varphi}{\calF}$ implies $\Satisfy{\varphi}{p}$.
% \end{definition}


% The subscript $v$ is ommitted whenever clear from context.
% \end{definition}

% \begin{definition}
% Conditions are interpreted as unary predicates:
% \begin{align*}
% \Interp{c} &: (\kw{FV}(c) \to \bbT) \to \calP(\bbT) \\
% \InterpA{\ctrivcst}{\varphi} &\triangleq \bbT \\
% \InterpA{\cequcst{T}}{\varphi} &\triangleq \Set{\InterpA{T}{\varphi}} \\
% \InterpA{\cgtcst{T}}{\varphi} &\triangleq \SetCmp{\tau \in \bbT}{\tau > \InterpA{T}{\varphi}} \\
% \InterpA{\cltcst{T}}{\varphi} &\triangleq \SetCmp{\tau \in \bbT}{\tau < \InterpA{T}{\varphi}} \\
% \InterpA{\clandcst{c_1}{c_2}}{\varphi} &\triangleq \InterpA{c_1}{\varphi} \cap \InterpA{c_2}{\varphi} \\
% \InterpA{\clorcst{c_1}{c_2}}{\varphi} &\triangleq \InterpA{c_1}{\varphi} \cup \InterpA{c_2}{\varphi}
% \end{align*}
% \end{definition}

% \begin{notation}
% When the assignment $\varphi$ is clear from context, 
% write $\tau \in c$ for the relation $\tau \in \InterpA{c}{\varphi}$
% \end{notation}

% \begin{definition}
% Define $\varphi \in \calF$ inductively over $\calF$: 
% \begin{align*}
%   [\,] \in \phi \quad &\text{iff} \quad \text{always} \\
%   \varphi[t \mapsto \tau] \in \calF, \IsOf{x}{c} \quad &\text{iff} \quad (\varphi \in \calF) \land (\tau \in c)
% \end{align*}
% \end{definition}

% \begin{definition}
% A tempral structure $\calM$ is a \emph{model} iff 
%  $\calF \entails{\IsOf{T}{c}}$ and $\varphi \in \calF$ implies 
% $\InterpA{T}{\varphi} \in \InterpA{c}{\varphi}$
% \end{definition}

% \begin{corollary}
% Given model $M$, if $\calF \entails{\eqcst{T_1}{T_2}}$ then 
% for all $\varphi \in \calF$, $\InterpA{T_1}{\varphi} = \InterpA{T_2}{\varphi}$.
% \end{corollary}

% \begin{corollary}
% Given model $M$, if $\calF \entails{\eqcst{D_1}{D_2}}$ then 
% for all $\varphi \in \calF$, $\InterpA{D_1}{\varphi} = \InterpA{D_2}{\varphi}$.
% \end{corollary}

% \begin{corollary}
% Given model $M$, elements of $\bbT$ admits trichotomy.
% \end{corollary}

% \emph{Remark.} Integers and real numbers are both models of this 
% calculus.
 

\subsection{Proof terms for multistep reduction relations}
% We introduce proof terms for the reduction relation. 

% Write $\boxed{\IsOf{\sigma}{\ClockProc{T}, \Omega \MultiStepsTo{} \ClockProc{T'}, \Omega'}}$ meaning 
% $\sigma$ witnesses a derivation deriving $\ClockProc{T}, \Omega \MultiStepsTo{} \ClockProc{T'}, \Omega'$.

% \begin{mathpar}
% \inferrule[]
% {\strut}
% {\IsOf{\StepRefl{T}{\Omega}}{\ClockProc{T}, \Omega \MultiStepsTo{} \ClockProc{T}, \Omega}}

% \inferrule[]
% {\leqcst{T_1}{T_2} \\
%   \IsOf{\sigma}{\ClockProc{T_2}, \Omega \MultiStepsTo{} \ClockProc{T_3}, \Omega'}}
% {\IsOf{\StepT{T_1}{T_2}{\Omega}{\sigma}}{\ClockProc{T_1}, \Omega \MultiStepsTo{} \ClockProc{T_3}, \Omega'}}

% \inferrule[]
% { \Omega \UStepsTo{T_1} \Omega' \\
%   \IsOf{\sigma}{\ClockProc{T_1}, \Omega' \MultiStepsTo{} \ClockProc{T_2}, \Omega''}}
% {\IsOf{\StepC{T_1}{\Omega}{\Omega'}{\sigma}}{\ClockProc{T_1}, \Omega \MultiStepsTo{} \ClockProc{T_2}, \Omega''}}
% \end{mathpar}

% A reduction relations $\ClockProc{T}, \Omega \MultiStepsTo{} \ClockProc{T'}, \Omega'$ therefore 
% induces a set of reductions sequences 
% $$
% (\ClockProc{T}, \Omega \MultiStepsTo{} \ClockProc{T'}, \Omega') \triangleq 
% \{\sigma \mid \IsOf{\sigma}{\ClockProc{T}, \Omega' \MultiStepsTo{} \ClockProc{T'}, \Omega'}\}$$

% \begin{definition}[Concatenation of Sequences]
% We define the \emph{concatenation} of $\sigma_1$ and $\sigma_2$:
% $$ 
% \concat{\cdot}{\cdot} : 
% (\ClockProc{T_0}, \Omega_0 \MultiStepsTo{} \ClockProc{T_1}, \Omega_1) \to 
% (\ClockProc{T_1}, \Omega_1 \MultiStepsTo{} \ClockProc{T_2}, \Omega_2) \to 
% (\ClockProc{T_0}, \Omega_0 \MultiStepsTo{} \ClockProc{T_2}, \Omega_2)
% $$

% The sequence $\concat{\sigma_1}{\sigma_2}$ is defined inductively over structure of $\sigma_1$ as follows:
% \begin{align*}
%   \concat{\StepRefl{T}{\Omega}}{\sigma_2}                  & \triangleq \sigma_2 \\
%   \concat{\StepC{T}{\Omega}{\Omega'}{\sigma_1}}{\sigma_2}  & \triangleq \StepC{T}{\Omega}{\Omega'}{\concat{\sigma_1}{\sigma_2}} \\
%   \concat{\StepT{T}{T'}{\Omega}{\sigma_1}}{\sigma_2}       & \triangleq \StepT{T}{T'}{\Omega}{\concat{\sigma_1}{\sigma_2}}
% \end{align*}
% \end{definition}

% The definition $\concat{\sigma_1}{\sigma_2}$ can then be extended to 
% $\IsOf{\sigma_1}{\ClockProc{T_0}, \Omega_0 \MultiStepsTo{} \ClockProc{T_1}, \Omega_1}$ \newline
% and $\IsOf{\sigma_2}{\ClockProc{T_1'}, \Omega_1 \MultiStepsTo{} \ClockProc{T_2}, \Omega_2}$
% with $T_1 \leq T_1'$, by setting 
% $$\concat{\sigma_1}{\sigma_2} \triangleq \concat{(\concat{\sigma_1}{\StepT{T_1}{T_1'}{\Omega_1}{\StepRefl{T_1'}{\Omega_1}}})}{\sigma_2}$$

% \begin{definition}[Interleaving of Sequences]
% We define the \emph{interleaving} of $\sigma_1$ and $\sigma_2$:
% $$ 
% \il{\cdot}{\cdot} : 
% (\ClockProc{T}, \Omega_1 \MultiStepsTo{} \ClockProc{T_1}, \Omega_1') \to 
% (\ClockProc{T}, \Omega_2 \MultiStepsTo{} \ClockProc{T_2}, \Omega_2') \to 
% (\ClockProc{T}, \conc{\Omega_1}{\Omega_2} \MultiStepsTo{} \ClockProc{\max(T_1, T_2)}, \conc{\Omega_1'}{\Omega_2'})
% $$

% The sequence $\il{\sigma_1}{\sigma_2}$ is defined inductively over the $\sigma_1$ and $\sigma_2$, 
% with the induction metric being the total length of both sequences as follows (symmetric cases are ommitted):
% \begin{align*}
%   \il{\StepRefl{T}{\Omega_1}}{\StepRefl{T}{\Omega_2}} 
%       & \triangleq \StepRefl{T}{\conc{\Omega_1}{\Omega_2}} \\
%   \il{\StepRefl{T}{\Omega_1}}{\StepC{T}{\Omega_2}{\Omega_2'}{\sigma_2}} 
%       & \triangleq \StepC{T}{(\Omega_1 \opconc \Omega_2)}{(\Omega_1 \opconc \Omega_2')}{\il{\StepRefl{T}{\Omega_1}}{\sigma_2}} \\
%   \il{\StepRefl{T}{\Omega_1}}{\StepT{T}{T'}{\Omega_2}{\sigma_2}} 
%       & \triangleq \StepT{T}{T'}{\conc{\Omega_1}{\Omega_2}}{\il{\StepRefl{T'}{\Omega_1}}{\sigma_2}} \\
%   \il{\StepC{T}{\Omega_1}{\Omega_1'}{\sigma_1}}{\StepC{T}{\Omega_2}{\Omega_2'}{\sigma_2}} 
%       & \triangleq 
%         \StepC{T}{\conc{\Omega_1}{\Omega_2}}{\conc{\Omega_1'}{\Omega_2}}{
%               \StepC{T}{\conc{\Omega_1'}{\Omega_2}}{\conc{\Omega_1'}{\Omega_2'}}{
%                 \il{\sigma_1}{\sigma_2}}}\\
%   \il{\StepC{T}{\Omega_1}{\Omega_1'}{\sigma_1}}{\StepT{T}{T'}{\Omega_2}{\sigma_2}} 
%       & \triangleq 
%           \StepC{T}{\conc{\Omega_1}{\Omega_2}}{\conc{\Omega_1'}{\Omega_2}}{
%             \StepT{T}{T'}{\conc{\Omega_1'}{\Omega_2}}{
%               \il{\sigma_1}{\sigma_2}
%             }} \\
%   \il{\StepT{T}{T_1}{\Omega_1}{\sigma_1}}{\StepT{T}{T_2}{\Omega_2}{\sigma_2}} 
%       & \triangleq 
%       \begin{cases*}
%               \StepT{T}{T_1}{\Omega_1, \Omega_2}{\il{\sigma_1}{\StepT{T_1}{T_2}{\Omega_2}{\sigma_2}}} 
%               & if $T_1 \leq T_2$ \\ 
%               \StepT{T}{T_2}{\Omega_1, \Omega_2}{\il{\StepT{T_2}{T_1}{\Omega_1}{\sigma_1}}{\sigma_2}} 
%               & if otherwise
%       \end{cases*}
% \end{align*}
% \end{definition}

% This definition can be extended to 
% $\IsOf{\sigma_1}{\ClockProc{T_1}, \Omega_1 \MultiStepsTo{} \ClockProc{T_1'}, \Omega_1'}$
% and $ \IsOf{\sigma_2}{\ClockProc{T_2}, \Omega_2 \MultiStepsTo{} \ClockProc{T_2'}, \Omega_2'}$ by:
% \begin{align*}
%   \il{\sigma_1}{\sigma_2} &: 
%     \ClockProc{\min(T_1, T_2)}, \conc{\Omega_1}{\Omega_2} \MultiStepsTo{} \ClockProc{\max{T_1'}{T_2'}}, \conc{\Omega_1'}{\Omega_2'} \\ 
%   \il{\sigma_1}{\sigma_2} &\triangleq 
%     \il{(\concat{\StepRefl{\min(T_1, T_2)}{\Omega_1}}{\concat{\sigma_1}{\StepRefl{\max(T_1', T_2')}{\Omega_2}}})}
%        {(\concat{\StepRefl{\min(T_1, T_2)}{\Omega_2}}{\concat{\sigma_2}{\StepRefl{\max(T_1', T_2')}{\Omega_2'}}})}
% \end{align*}


\subsection{Functions over temporal intervals}

% \begin{definition}[Temporal Intervals]
% A temporal interval $I$ is either \emph{bounded} or \emph{unbounded}: 
% \begin{itemize}
%   \item (Bounded) $\TInt{\tau_1}{\tau_2} \triangleq \SetCmp{ \tau \in \bbT}{\tau_1 \leq \tau < \tau_2}$
%   \item (Unbounded) $\TIntInf{\tau} \triangleq \SetCmp{\tau' \in \bbT}{\tau \leq \tau'}$
% \end{itemize}
% \end{definition}

% \begin{notation}
% Let $T_1$, $T_2$ and $T$ be closed elemetns of sort $\Sort{Time}$. 
% Define $\TInt{T_1}{T_2} \triangleq \TInt{\Interp{T_1}}{\Interp{T_2}}$; 
% define $\TIntInf{T} \triangleq \TIntInf{\Interp{T}}$; 
% \end{notation}

% \begin{notation}
% Given closed $T$ and interval $I$, define $T \in I$ meaning $\Interp{T} \in I$.
% \end{notation}

% \begin{notation}
% Given a fixed $I$, we will use $I = \TInt{\tau_1}{\tau_2}$ to extract the end points of an interval, with the understanding that only $\tau_1$ is 
% bounded to a point in time if the $I$ is unbounded. In this case we may informally say $\tau_2 = \infty$.
% \end{notation}

% We are particularly interested in \emph{configuration-valued functions on intervals}. These functions depicts a trajectory
% of evolution for a configuration over a period of time.

% \begin{definition}
% A \emph{trajectory} is function $I \to \Sort{Conf}$. 
% Let $r$ be a trajectory, if its domain $I$ is unbounded then it is said to be \emph{a world line}, 
% otherwise it is said to be a \emph{world line segment}. 
% The set of trajectories over interval $I$ is denoted $\Trj{I}$.
% \end{definition}

% Among all trajectories, we name a few notable ones:

% \begin{definition}
% Given an empty interval $I$ (that is, $I = \emptyset$). Let $\trjTriv{I}$ denote the trivial function over it. 
% In particular, let $\trjTriv{\tau}$ denote the trivial function on the (empty) interval $\TInt{\tau}{\tau}$.
% \end{definition}

% \begin{definition}
% Given an interval $I$ and some configuration $\Omega$. Let $\trjConst{I}{\Omega}$ denote the constant function on $I$: 
% $$\trjConst{I}{\Omega} : I \to \Sort{Conf} \triangleq t \mapsto \Omega$$
% \end{definition}

% We may define operators on trajectories:

% \begin{definition}
% The \emph{concatenation} operation stitches two world lines (segments) with adjacent domains: 
% \begin{align*}
%   \trjCat{\cdot}{\cdot} &: \Trj{\TInt{\tau_1}{\tau_2}} \times \Trj{\TInt{\tau_2}{\tau_3}} \to \Trj{\TInt{\tau_1}{\tau_3}} \\
%   \trjCat{r}{s} &\triangleq t \mapsto
%         \begin{cases*}
%           r(t) & $t \in \TInt{\tau_1}{\tau_2}$ \\
%           s(t) & $t \in \TInt{\tau_2}{\tau_3}$ 
%         \end{cases*}
% \end{align*}
% \end{definition}

% \begin{definition}
% The following operator extends the domain of $r : \Trj{\TInt{\tau_1}{\tau_2}}$ to $\TInt{\tau_0}{\tau_2}$ by a constant.
% $$\trjExt{\tau_0}{\Omega}{r} \triangleq \trjCat{\trjConst{\TInt{\tau_0}{\tau_1}}{\Omega}}{r}$$
% \end{definition}

% \begin{definition}
% The \emph{interleaving} of two world lines (segments) (on the same domain) pointwise parallel composes configurations:
% \begin{align*}
%   \trjConc{\cdot}{\cdot} &: \Trj{\TInt{\tau_1}{\tau_2}} \times \Trj{\TInt{\tau_1}{\tau_2}} \to \Trj{\TInt{\tau_1}{\tau_2}} \\
%   \trjConc{r}{s} &\triangleq t \mapsto \conc{r(t)}{s(t)}
% \end{align*}
% \end{definition}

\subsection{Computable World Lines and Segments}

% We are overloading names (and symbols) for the operators. In most contexts, it should be immediately clear 
% by examining the type of the arguments. The choice to overload them is intentional: operations on world lines 
% (segments) reflects by operations on reduction sequences in a precise sense, as we will see now.

% A world line (segment) is said to be \emph{computable} if it can be ``explained'' by a reduction sequence.
% This is formally setup as binary relation between world line (segments) and reductions sequences, defined 
% with inference rules. 


% Let $\computes{\sigma}{f}$ be the strongest relation $\Rel{\sigma}{r}$ satisfying: 

% \begin{itemize}
%   \item $\Rel{\StepRefl{T}{\Omega}}{\trjConst{\TInt{\tau}{\tau'}}{\Omega}}$ iff $\tau = \Interp{T}$ and $\tau' \geq \tau$.
%   \item $\Rel{\StepC{T}{\Omega}{\Omega'}{\sigma}}{r}$ iff $\computes{\sigma}{r}$.
%   \item $\Rel{\StepT{T}{T'}{\Omega}{\sigma}}{\trjExt{\Interp{T}}{\Omega}{r}}$ iff $\computes{\sigma}{r}$.
% \end{itemize}

% \begin{mathpar}
% \inferrule
% {\strut}
% {\computes{\StepRefl{T}{\Omega}}{\trjConst{\TInt{\tau}{\tau'}}{\Omega}}}

% \inferrule
% {\computes{\StepC{T}{\Omega}{\Omega'}{\sigma}}{r}}

% \inferrule
% {\computes{\sigma}{r}}
% {\computes{\StepT{T}{T'}{\Omega}{\sigma}}{\trjExt{T}{\Omega}{r}}}
% \end{mathpar}

% We now now define two functions $\computewls{\cdot}$ and  $\computewl{\cdot}$ mapping reduction sequence 
% into world lines segments and world lines respectively. A world line (segment) is therefore 
% said to be \emph{computable} if it is the image of some reduction sequence by this function.

% \begin{definition}
% We are to define the following two functions:
% \begin{align*}
% \IsOf{\computewls{\cdot}}{(\ClockProc{T}, \Omega \MultiStepsTo{} \ClockProc{T'}, \Omega') \to (\TInt{T}{T'} \to \Sort{Conf})} \\
% \IsOf{\computewl{\cdot}}{(\ClockProc{T}, \Omega \MultiStepsTo{} \ClockProc{T'}, \Omega') \to (\TIntInf{T} \to \Sort{Conf})}
% \end{align*}
% Define $\computewls{\cdot}$ over the structure of input:
% \begin{align*}
%   \computewls{\StepRefl{T}{\Omega}}               &\triangleq \text{undefined}\\
%   \computewls{\StepC{T}{\Omega}{\Omega'}{\sigma}} &\triangleq t \mapsto \computewls{\sigma}(t)\\
%   \computewls{\StepT{T}{T'}{\Omega}{\sigma}}     &\triangleq t \mapsto 
%   \begin{cases*}
%               \Omega                 & $ t \in \TInt{T}{T'}$  \\
%               \computewls{\sigma}(t) & if otherwise
%   \end{cases*}
% \end{align*}
% \end{definition}

% Define $\computewl{\cdot}$ by extending the domain of $\computewls{\cdot}$: 
% $$
% \computewl{\sigma} \triangleq 
%   \begin{cases*}
%         \computewls{\sigma}(t) & $t \in \TInt{T}{T'}$ \\
%         \Omega'                & $t \in \TIntInf{T'}$
%   \end{cases*}
% $$

% The definition is well-formed as in the closed instance of $T$, as it admits trichotomy.

% The setup finally culminates in the following definition:

% \begin{definition}
% Given $\IsOf{\sigma}{\ClockProc{T}, \Omega \MultiStepsTo{} \ClockProc{T'}, \Omega'}$, and a 
% trajectory $r$. If $r$ is a world line then the pair is a \emph{computable world line}; 
% if $r$ is a world line segment then the pair is a \emph{computable world line segment}.
% \end{definition}

% The pair $\pairexcst{r}{\sigma}$ is a \emph{computable trajectory} 
% iff $\computes{\sigma}{r}$. The the domain of $r$ is said to be the \emph{domain} of the trajectory. 
% The configuration $\Omega$ is said to be the \emph{initial configuration}.
% If domain is unbounde then $\Omega'$ is said to be the \emph{terminal configuration} of the computable world line segment.


\begin{definition}
Let $w \in \ctrj{\tau_1}{\tau_2}{\Omega}{\Omega'}$ denote a computable trajectory 
with domain $\TInt{\tau_1}{\tau_2}$ and initial and terminal configuration (if exists) 
being $\Omega$ and $\Omega'$ respectively. 

In the case that $w$ is world line segment, $\tau_2$ is formally written as $\infty$ and $\Omega'$ is represented
by an underscore. We may also drop both (i.e. write just $w \in \cwl{\tau_1}{\Omega}$) for emphasis.
\end{definition}

% \begin{definition}
% Let $w = \pairexcst{r}{\sigma}$ be a computable world trajectory with domain $I$. 
% Define for all $\tau \in I$, $w(\tau) \triangleq r(\tau)$ for the configuration \emph{at} time $\tau \in I$.
% \end{definition}

% \begin{definition}
% For all configurations $\Omega$, there is a trivial trajecotry on interval $\TInt{T_1}{T_2}$, defined as
% $\constcwl{\TInt{T_1}{T_2}}{\Omega} \triangleq \pairexcst{\trjConst{\TInt{T_1}{T_2}}{\Omega}}{\StepRefl{T_1}{\Omega}}$.
% \end{definition}

\subsection{Operations on and properties of computable trajectories}

% \begin{definition}[Equivalence]
% Trajectories $w_1 \in \ctrjI{I_1}{\Omega_1}{\Omega_1'}$ and $w_2 \in \ctrjI{I_2}{\Omega_2}{\Omega_2'}$
% are said to be \emph{equivalent} on interval $I$, $\cwlequivt{I}{w_1}{w_2}$, 
% iff for all $\tau \in I$, $w_1(\tau) = w_2(\tau)$. 
% In particular, if $I = I_1 = I_2$ and $\cwlequivt{I}{w_1}{w_2}$ (i.e. their domains coincide and they are equivalent 
% on the entire domain), write just $\cwlequiv{w_1}{w_2}$.
% \end{definition}

% \begin{definition}[Equivalence]
% Let $w_1 \in \cwl{T_1}{\Omega_1}$ and $w_2 \in \cwl{T_2}{\Omega_2}$. If for all $\IsOf{T'}{\cgeqcst{T}}$, 
% $w_1(T') = w_2(T')$ (both has to be well-defined), then $w_1$ is equivalent to $w_2$ after $T$, denoted by
% $\cwlequivt{T}{w_1}{w_2}$.
% \end{definition}


Easy to verify that this define an equivalence relation.

% \begin{definition}[Concatenation]
% Let $w_1 = \pairexcst{r}{\sigma} \in \ctrj{\tau_1}{\tau_2}{\Omega}{\Omega'}$ be a segment 
% and $w_2 = \pairexcst{s}{\sigma'} \in \ctrj{\tau_2}{\tau_3}{\Omega'}{\Omega''}$ be a trajectory. 
% Define the \emph{concatenation} of $w_1$ and $w_2$, 
% as $\concat{w_1}{w_2} \triangleq \pairexcst{\trjCat{r}{s}}{\concat{\sigma}{\sigma'}}$.
% Further more, $\cwlequivt{\TInt{\tau_1}{\tau_2}}{(\concat{w_1}{w_2})}{w_1}$ and 
% $\cwlequivt{\TInt{\tau_2}{\tau_3}}{(\concat{w_1}{w_2})}{w_2}$.
% \end{definition}
% \begin{proof}
% \emph{(Incomplete)} We need to show that $\computes{\concat{\sigma}{\sigma'}}{\trjCat{l}{g}}$. 
% \end{proof}

% \begin{lemma}
% For all $w$ and $s$ in the definition, $\cwlequivt{\TIntInf{T}}{(\concat{s}{w})}{w}$.
% \end{lemma}
% \begin{proof}
% Directly from definition. 
% \end{proof}

% A worldline $w \in \cwl{T}{\Omega}$ describes the trajectory of $\Omega$ for all time 
% later than $T$. It should be able to pick a time $T'$ in the future $T$ and obtain a 
% worldline $w' \in \cwl{T'}{\Omega'}$ by cutting off the segment between $T'$ and $T$. 
% This operation can be viewed as a dual to the extension operation. This motivates the 
% following definition: 

% \begin{definition}
% Given $w = \pairexcst{l}{\sigma} \in \cwl{T}{\Omega}$, for all $T' \in \TIntInf{T'}$, 
% a line $w' \in \cwl{T'}{w(T')}$ is said to be the cuff said
% \end{definition}

% \begin{definition}[Partition]
% Given $w = \pairexcst{r}{\sigma}\in \ctrj{\tau_1}{\tau_2}{\Omega}{\Omega'}$ be a trajectory, 
% for all $T$ such that $\Interp{T} \in \TInt{\tau_1}{\tau_2}$, 
% the \emph{partitions} of $w$ at $\tau$ is a pair of trajectories: 
% \begin{itemize}
%   \item the \emph{left partition} $\lpar{w}{T} \in \ctrj{\tau_1}{\Interp{T}}{\Omega}{w(\tau)}$, and
%   \item the \emph{right partition} $\rpar{w}{T} \in \ctrj{\Interp{T}}{\tau_2}{w(\tau)}{\Omega'}$,
% \end{itemize}
% such that $\cwlequiv{w}{\concat{(\lpar{w}{T})}{(\rpar{w}{T})}}$,

% Both are defined inductively over $\sigma$:
% \bgroup
% \NewDocumentCommand{\PiOne}{m}{\pi_1({#1})}
% \NewDocumentCommand{\PiTwo}{m}{\pi_2({#1})}
% \begin{align*}
%   \lpar{\pairexcst{\trjConst{\TInt{\tau_1}{\tau_2}}{\Omega}}{\StepRefl{T_1}{\Omega}}}{T} 
%     &\triangleq \pairexcst{\trjConst{\TInt{\tau_1}{\Interp{T}}}{\Omega}}{\StepRefl{T_1}{\Omega}} \\
%   \rpar{\pairexcst{\trjConst{\TInt{\tau_1}{\tau_2}}{\Omega}}{\StepRefl{T}{\Omega}}}{T} 
%     &\triangleq \pairexcst{\trjConst{\TInt{\Interp{T}}{\tau_2}}{\Omega}}{\StepRefl{T}{\Omega}} \\
%   \lpar{\pairexcst{r}{\StepC{T_1}{\Omega}{\Omega'}{\sigma}}}{T} 
%     &\triangleq \pairexcst{r'}{\StepC{T_1}{\Omega}{\Omega'}{\sigma'}} 
%       \text{ where } \pairexcst{r'}{\sigma'} = \lpar{\pairexcst{r}{\sigma}}{T} \\
%   \rpar{\pairexcst{r}{\StepC{T_1}{\Omega}{\Omega'}{\sigma}}}{T} &\triangleq \rpar{\pairexcst{r}{\sigma}}{T}\\
%   \lpar{\pairexcst{\trjExt{\tau_1}{\Omega}{r}}{\StepT{T_1}{T_1'}{\Omega}{\sigma}}}{T}  
%     &\triangleq 
%     \begin{cases*}
%               \pairexcst{\trjConst{\TInt{\tau_1}{\Interp{T}}}{\Omega}}{\StepT{T_1}{T}{\Omega}{\StepRefl{T}{\Omega}}}
%               & if $\Interp{T} \in \TInt{\tau_1}{\Interp{T_1'}}$ \\
%               \pairexcst{\trjExt{\tau_1}{\Omega}{r'}}{\StepT{T}{T_1'}{\Omega}{\sigma'}}
%               \text{ where } \pairexcst{r'}{\sigma'} = \lpar{\pairexcst{r}{\sigma}}{T}
%               & if $\Interp{T} \in \TInt{\Interp{T_1'}}{\tau_2}$ 
%     \end{cases*} \\
%   \rpar{\pairexcst{\trjExt{\tau_1}{\Omega}{r}}{\StepT{T_1}{T_1'}{\Omega}{\sigma}}}{T}  
%     &\triangleq 
%     \begin{cases*}
%               \pairexcst{\trjExt{\tau_1}{\Omega}{r'}}{\StepT{T_1}{T_1'}{\Omega}{\sigma'}}
%               \text{ where } \pairexcst{r'}{\sigma'} = \rpar{\pairexcst{r}{\sigma}}{T}
%               & if $\Interp{T} \in \TInt{\tau_1}{\Interp{T_1}}$ \\
%               \rpar{\pairexcst{r}{\sigma}}{T}   
%               & if $\Interp{T} \in \TInt{\Interp{T_1'}}{\tau_2}$
%     \end{cases*}
% \end{align*}
% \egroup
% \end{definition}

% \emph{Remark.} Partitioning could, and arguably should have defined for all $\tau \in \TInt{\tau_1}{\tau_2}$, 
% but this requires the dynamics to be stated for a particular choice of model instead of syntactic objects.

% \begin{lemma}
% For $w$ and $T'$ in above definition, $\cwlequivt{\TIntInf{T'}}{w}{\cutoff{w}{T'}}$.
% \end{lemma}
% \begin{proof}
% Fix arbitrary $t \in \TIntInf{T'}$, the goal is to show that $w(t) = \cutoff{w}{T'}(t)$. Expand the definition for the cutoff and proceed
% by case analysis. In the first case both sides are just $\Omega$. In the second case and the first subcase of the third case, 
% directly appeal to inductive hypothesis. In the final case, remark that $\trjExt{T}{\Omega}{l}(t) = \Omega = \trjExt{T'}{\Omega}{l}(t)$ 
% if $t \in \TInt{T'}{T''}$, and otherwise appeal to in the inductive hypothesis.
% \end{proof}

% Cut-offs and extensions are dual in the sense of the following lemma.

% \begin{lemma}
% For all $w \in \cwl{\Omega}{T}$, then:
% \begin{enumerate}
%   \item For all $\IsOf{s}{\cwls{T'}{T}{\Omega'}{\Omega}}$, 
%   then $\cwlequiv{w}{\cutoff{(\concat{s}{w})}{T}}$.
%   \item Let $s$ witness the cut-off $\cutoff{w}{T'}$, then $\cwlequiv{w}{\concat{s}{\cutoff{w}{T'}}}$.
% \end{enumerate}
% \end{lemma}
% \begin{proof}
% To show the first theorem, note that $\cwlequivt{T}{\concat{s}{w}}{w}$, and 
% $\cwlequivt{T}{\cutoff{(\concat{s}{w})}{T}}{\concat{s}{w}}$, conclude by symmetry and transitivity. The argument is 
% Essentially identical for the second one and left as an exercise.
% \end{proof}

% Up until this point the operations we investigated are done along a singular trajectory. Processes in a system 
% runs in parallel: each individual process has an associate associated, and the whole system also has a trajectory 
% that determined pointwise for every instant by the individual component trajectory.

% \begin{definition}[Interleaving computable trajectories]
% The \emph{interleaving} operator on trajectories is defined as follows:
% \begin{align*}
%   \il{\cdot}{\cdot} &:
% \ctrj{\tau}{\tau'}{\Omega_1}{\Omega_1'} \to 
% \ctrj{\tau}{\tau'}{\Omega_2}{\Omega_2'} \to
% \ctrj{\tau}{\tau'}{\conc{\Omega_1}{\Omega_1'}}{\conc{\Omega_2}{\Omega_2'}} \\
% \il{\pairexcst{r_1}{\sigma_1}}{\pairexcst{r_2}{\sigma_2}} &\triangleq
% \pairexcst{\trjConc{r_1}{r_2}}{\il{\sigma_1}{\sigma_2}}
% \end{align*}
% \end{definition}

% \begin{lemma}
% For all $w_1 \in \cwl{T}{\Omega_1}$ and $w_2 \in \cwl{T}{\Omega_2}$,
% $(\il{w_1}{w_2})(t) = \conc{w_1(t)}{w_2(t)}$.
% \end{lemma}

% \begin{lemma}
% The interleaving operation $\il{w_1}{w_2}$ is symmetric, associative and conguerent with respect 
% to the equivalence on computable worldlines:
% \begin{itemize}
%   \item (Symmetry) $\cwlequiv{\il{w_1}{w_2}}{\il{w_1}{w_2}}$
%   \item (Associativity) $\cwlequiv{\il{(\il{w_1}{w_2})}{w_3}}{\il{w_1}{(\il{w_2}{w_3})}}$
%   \item (Congurence) If $\cwlequiv{w_1}{w_1'}$ and $\cwlequiv{w_2}{w_2'}$, then $\cwlequiv{\il{w_1}{w_2}}{\il{w_1'}{w_2'}}$
% \end{itemize}
% \end{lemma}
% \begin{proof}
% Straightforward from definition.
% \end{proof}

% We now investigate how interleaving interacts with extension and cutting-off.

% \begin{lemma}
% For all $w_1 \in \ctrjI{I}{\Omega_1}{\Omega_1'}$ and $w_2 \in \ctrjI{I}{\Omega_2}{\Omega_2'}$ 
% and for all $T \in I$, 
% \begin{itemize}
%   \item $\cwlequiv{\lpar{(\il{w_1}{w_2})}{T}}{\il{(\lpar{w_1}{T})}{(\lpar{w_2}{T})}}$.
%   \item $\cwlequiv{\rpar{(\il{w_1}{w_2})}{T}}{\il{(\rpar{w_1}{T})}{(\rpar{w_2}{T})}}$.
%   \item $\cwlequiv{\concat{(\il{\lpar{w_1}{T}}{\lpar{w_2}{T}})}{(\il{\rpar{w_1}{T}}{\rpar{w_2}{T}})}}
%                   {\il{w_1}{w_2}}$
% \end{itemize}
% \end{lemma}
% \begin{proof}
% By direct computation.
% \end{proof}
% \begin{proof}
% For all suitable $T''$, $((\cutoff{(\il{w_1}{w_2})}{T'})(T'')) = (\il{w_1}{w_2})(T'') = \conc{w_1(T'')}{w_2(T'')}$.

% On the other hand, $(\il{(\cutoff{w_1}{T'})}{(\cutoff{w_2}{T'})})(T'') = \conc{(\cutoff{w_1}{T'}(T''))}{(\cutoff{w_2}{T'}(T''))} = \conc{w_1(T'')}{w_2(T'')}$.
% \end{proof}

% \begin{lemma}
% Let $w_1 \in \cwl{T}{\Omega_1}$ and $w_2 \in \cwl{T}{\Omega_2}$. 
% Let $s_1 \in \cwls{T'}{T}{\Omega_1'}{\Omega_1}$ and 
% $s_2 \in \cwls{T'}{T}{\Omega_2'}{\Omega_2}$. 
% Then $\cwlequiv{\concat{(\il{s_1}{s_2})}{(\il{w_1}{w_2})}}{\il{(\concat{s_1}{w_1})}{(\concat{s_2}{w_2})}}$.
% \end{lemma}
% \begin{proof}
% Fix any $t \in \TIntInf{T'}$: 
% \begin{itemize}
%   \item If $t \in \TIntInf{T}$ then $(\concat{(\il{s_1}{s_2})}{(\il{w_1}{w_2})})(t) = (\il{w_1}{w_2})(t) = \conc{w_1(t)}{w_2(t)}$.

%   On the other hand $\il{(\concat{s_1}{w_1})}{(\concat{s_2}{w_2})}(t) = 
%   \conc{(\concat{s_1}{w_1})(t)}{(\concat{s_2}{w_2})(t)} = \conc{w_1(t)}{w_2(t)}$

%   \item Otherwise $t \in \TInt{T}{T'}$ then
%   $(\concat{(\il{s_1}{s_2})}{(\il{w_1}{w_2})})(t) = (\il{s_1}{s_2})(t) = \conc{s_1(t)}{s_2(t)}$.

%   On the other hand $\il{(\concat{s_1}{w_1})}{(\concat{s_2}{w_2})}(t) = 
%   \conc{(\concat{s_1}{w_1})(t)}{(\concat{s_2}{w_2})(t)} = \conc{s_1(t)}{s_2(t)}$
% \end{itemize}
% \end{proof}

% \begin{lemma}
% For all $w_1 \in \cwl{T}{\Omega_1}$ and $w_2 \in \cwl{T}{\Omega_2}$ and for all suitable $T'$, 
% let $s_1$ witness $\cutoff{w_1}{T'}$ and $s_2$ witness $\cutoff{w_2}{T'}$. 
% Then $\cwlequiv{\il{w_1}{w_2}}{\concat{(\il{s_1}{s_2})}{(\il{\cutoff{w_1}{T'}}{\cutoff{w_2}{T'}})}}$.
% \end{lemma}
% \begin{proof}
% Compute 
% $\cwlequiv{\concat{(\il{s_1}{s_2})}{(\il{\cutoff{w_1}{T'}}{\cutoff{w_2}{T'}})}}{
%   \cwlequiv{\il{(\concat{s_1}{\cutoff{w_1}{T'}})}{(\concat{s_2}{\cutoff{w_2}{T'}})}}{\il{w_1}{w_2}}}$
% \end{proof}
 
\subsection{Logical relations}

Define an auxilary sort of \emph{exposed types} $\mathcal{A}$ as follows: 
$$ \calA ::= \unitstycst \mid \tensorstycst{A_1}{A_2} \mid \larrstycst{A_1}{A_2} \mid \bsumstycst{A_1}{A_2} \mid \bwithstycst{A_1}{A_2}$$

Take note that the definition is not recursive: the component types (if any) are regular realtime-temporal session types.

We can $\emph{expose}$ a temporal type $A$ at some point in time $T$, resulting and exposed type. 
Let $\expose{A}{T}$ stand for the exposed type of $A$ at time $T$. It is defined as follows: 
\begin{align*}
  \expose{\tpunitstycst{t}{p}}{T}                  &\triangleq \unitstycst \\
  \expose{(\tptensorstycst{t}{p}{A_1}{A_2})}{T} &\triangleq \tensorstycst{(\Subst{T}{t}{A_1})}{(\Subst{T}{t}{A_2})}\\
  \expose{(\tplarrstycst{t}{p}{A_1}{A_2})}{T}   &\triangleq \larrstycst{(\Subst{T}{t}{A_1})}{(\Subst{T}{t}{A_2})}\\
  \expose{(\tpsumstycst{t}{p}{A_1}{A_2})}{T}   &\triangleq \bsumstycst{(\Subst{T}{t}{A_1})}{(\Subst{T}{t}{A_2})}\\
  \expose{(\tpwithstycst{t}{p}{A_1}{A_2})}{T}  &\triangleq \bwithstycst{(\Subst{T}{t}{A_1})}{(\Subst{T}{t}{A_2})}
\end{align*}

\begin{notation}
In contexts that are clear, we write $\wp{A}{p}{t}$ in place of the meta-variable $A$, where 
$p(t)$ pattern matches the predicate associated with the top-level connective. 
\end{notation}

Our logical predicate differentiate itself from tradition in that it's define for pairs $\gl{\bfw}{\bfOmega}$, 
call \emph{temporal computability pairs},
where the components are \emph{(runtime) channel indexed families} of computable world lines (from some fixed time $\tau$)
and configurations, satisfying $\bfw_a \in \cwl{\tau}{\bfOmega_a}$ for all indicies $a$. This condition is then 
denoted by $\bfw \in \cwl{\tau}{\bfOmega}$.

The logical predicate is defined mutual inductively over $A$. Our development defines four related predicates:
\begin{align*}
  \gl{\bfw}{\bfOmega} \in \LSInt{A}{T} & \quad \text{Interpreting \emph{latent} configurations in context with evidence $w$.} \\
  \bfOmega \in \VSInt{\calA}{T} & \quad \text{Interpreting \emph{visible} configuration in context.} \\
  \gl{\bfw}{\bfOmega} \in \LInt{A}{T}  & \quad \text{Interpreting \emph{latent} configuration as provider with evidence $w$.} \\
  \bfOmega \in \VInt{\calA}{T}  & \quad \text{Interpreting \emph{visible} configuration as provider.} 
\end{align*}  

Intuitively $\gl{\bfw}{\bfOmega} \in \LSInt{A}{T}$ means that $\bfw_a \in \cwl{\tau}{\bfOmega_a}$ supports, or is the evidence for, 
$\bfOmega_a$ being a member within the interpretation at all indicies. 

Above definitions generalize to contexts as follows: 

% \begin{definition}[$\gl{\bfw}{\bfOmega}_x \in \LSInt{\Delta}{T}$]
% Let $\IsOf{\gamma}{\Delta \leftrightarrow \Sigma}$ witness a bijection between a set of (runtime) 
% channels $\Sigma$ and entries of context $\Delta$. Let $w_a$ and $\Omega_a$ be families of 
% world lines and configurations indexed by $\Sigma$. We say $\gl{w_a}{\Omega_a} \in \LSInt{\Delta}{T}$ iff

% \begin{itemize}
%   \item For all $(\IsOf{x}{A}) \in \Delta$, $\gl{w_{\gamma(x)}}{\Omega_{\gamma(x)}} \in \LSInt{A}{T}$, or equivalently 
%   \item For all $a \in \Sigma$, $\gl{w_a}{\Omega_a} \in \LSInt{\Delta_{\gamma^{-1}(a)}}{T}$
% \end{itemize}
% \end{definition}
\begin{definition}
A \emph{concurrent composition} for $\Delta$ is a map from $\Delta$ to temporal computability pairs, denoted by $\delta$.
\end{definition}

\begin{definition}[$\delta \in \LSInt{\Delta}{T}$]
Define $\delta \in \LSInt{\Delta}{T}$ iff for all $(\IsOf{x}{A}) \in \Delta$, $\delta_x \in \LSInt{A}{T}$
\end{definition}

\begin{definition}
A \emph{(runtime) channel substitution} for $\Delta$ is a map from $\Delta$ to channels, denoted by $\gamma$.
\end{definition}

% In the following development, in contexts where $\gamma$ is clear (but might be implicit), 
% we will write $w_x$ for $w_{\gamma(x)}$ and $\Delta_a$ for $\Delta_{\gamma^{-1}(a)}$. 
% Write $a \in \Delta$ for $a \in \gamma^{-1}(\Delta)$.

% From there we build auxilary definitions:

\begin{definition}[$\Delta \sementails{\IsOfProc{P}{T}{A}}$]
For all $\delta \in \LSInt{\Delta}{T}$ and for all channel substitutions $\eta$,
$\exists w$ such that $\gl{w}{\conc{(\ilfam{x \in \Delta}{\bfOmega^x_{\eta(x)}})}{\RunProc{a}{\hat{\eta}(P)}}} \in \LInt{A}{T}$.
\end{definition}

\begin{definition}
Given $\calG \entails{\IsCtx{\calF}}$, let $\varphi$ be a map (i.e. substitution) from $\Sort{Time}$ to $\calG$.
Write $\varphi \in (\calG; \calF)$ (or just $\varphi \in \calF$ when $\calG$ is clear from context)
for $\Satisfy{\Interp{\varphi}}{\calF}$, where $\Interp{\varphi}$ applies interpretation function 
pointwise.
\end{definition}

\begin{definition}[$\calG; \calF \mid \Delta \sementails{\IsOfProc{P}{T}{A}}$]
For all $\varphi \in \calF$, 
$\hat{\varphi}(\Delta) \sementails{\IsOfProc{\hat{\varphi}(P)}{\hat{\varphi}(T)}{\hat{\varphi}(A)}} $  \\
\end{definition}

\begin{notation}
Given a predicate $p(t)$ (i.e. an element of sort $\Sort{Prop}$ with a single distinguished free temporal variable $t$) 
 and an element $T$ of sort $\Sort{Time}$, write $\Satisfy{t}{p}$ for $\Satisfy{[t \mapsto \Interp{T}]}{p}$.
\end{notation}

Definitions for cases of the logical relations:

\newcolumntype{L}{>$l<$}
\newcolumntype{C}{>$c<$}
\begin{tabular}{lcp{\textwidth}}
$\gl{\bfw}{\bfOmega} \in \LSInt{\wp{A}{p}{t}}{T}$ & iff &
  For all $t$ s.t. $\Satisfy{t}{p}$, then $\bfw(t) \in \VSInt{\expose{A}{t}}{t}$. \\
\\
$\gl{\bfw}{\bfOmega} \in \LInt{\wp{A}{p}{t}}{T}$ & iff & 
  For all $t$ s.t. $\Satisfy{t}{p}$, then $\Interp{t} \geq \Interp{T}$ and $\bfw(t) \in \VInt{\expose{A}{t}}{t}$. \\
\\
$\bfOmega \in \VAnyInt{\unitstycst}{T}$ & iff & 
  $\bfOmega = \RunProc{a}{\tpclosecst{t}{p}}$ for some $p$ and $\Satisfy{T}{p}$. \\
\\
$\bfOmega \in \VAnyInt{\bwithstycst{A_1}{A_2}}{T}$ & iff & 
  $\bfOmega = \RunProc{a}{\tpoffercst{t}{p}{P_1}{P_2}} \opconc \Omega'$,  
  for some $\Omega'$ and $p$ such that $\Satisfy{T}{p}$:
  \begin{itemize}
    \item $\exists{\bfw_1}$, $\gl{\bfw_1}{(\RunProc{a}{\Subst{T}{t}{P_1}} \opconc \Omega')} \in \LAnyInt{A_1}{T}$, and  
    \item $\exists{\bfw_2}$, $\gl{\bfw_2}{(\RunProc{a}{\Subst{T}{t}{P_2}} \opconc \Omega')} \in \LAnyInt{A_2}{T}$.
  \end{itemize}\\

$\bfOmega \in \VAnyInt{\bsumstycst{A_2}{A_2}}{T}$ & iff & Either
  (for some $p$ and $\Satisfy{T}{p}$),
  \begin{itemize}
    \item $\bfOmega_a = \RunProc{a}{\tpinlcst{t}{p}{A_1}{A_2}{P}} \opconc \Omega'$ and 
          $\exists \bfw$, $\gl{\bfw}{(\RunProc{a}{\Subst{T}{t}{P}} \opconc \Omega')} \in_a \LAnyInt{A_1}{T}$, or  
    \item $\bfOmega_a = \RunProc{a}{\tpinrcst{t}{p}{A_1}{A_2}{P}} \opconc \Omega'$ and 
          $\exists \bfw$, $\gl{\bfw}{(\RunProc{a}{\Subst{T}{t}{P}} \opconc \Omega') \in_a \LAnyInt{A_2}{T}}$.
  \end{itemize}\\

$\bfOmega \in \VAnyInt{\tensorstycst{A_1}{A_2}}{T}$ & iff &
   $\bfOmega = \RunProc{a}{\tptensorsndcst{t}{p}{P_1}{P_2}} \opconc \Omega_1 \opconc \Omega_2$ 
  for some $p$ and $\Satisfy{T}{p}$, s.t. 
  \begin{itemize}
    \item $\exists \bfw_1$, $\gl{\bfw_1}{(\RunProc{a}{\Subst{T}{t}{P_2}} \opconc \Omega_2)} \in_a \LAnyInt{A_2}{T}$, and
    \item $\exists \bfw_2$, $\gl{\bfw_2}{(\RunProc{a}{\Subst{T}{t}{P_1}} \opconc \Omega_1)} \in_b \LAnyInt{A_1}{T}$.
  \end{itemize}\\

$\bfOmega \in \VInt{\larrstycst{A_1}{A_2}}{T}$ & iff &
   $\bfOmega = \RunProc{a}{\tplarrrcvcst{t}{p}{x}{P}} \opconc \Omega_2$ for 
   some $p$ and $\Satisfy{T}{p}$, s.t. \newline
   $\forall \gl{\bfw_1}{\bfOmega_1} \in \LSInt{A_1}{T}$, \newline
   $\forall b$, $\exists \bfw_2$, $\gl{\bfw_2}{(\RunProc{a}{\Subst{T, b}{t, x}{P}} \opconc \bfOmega_1(b) \opconc \Omega_2)} \in_a \LInt{A_2}{T}$. \\

$\bfOmega \in \VSInt{\larrstycst{A_1}{A_2}}{T}$ & iff &
   $\bfOmega = \RunProc{a}{\tplarrrcvcst{t}{p}{x}{P}} \opconc \Omega_2$ 
   for some $p$ and $\Satisfy{T}{p}$ s.t. \newline
   $\forall \gl{\bfw_1}{\bfOmega_1} \in_b \LInt{A_1}{T}$, \newline
   $\forall b$, $\exists \bfw_2$, $\gl{\bfw_2}{(\RunProc{a}{\Subst{T, b}{t, x}{P}} \opconc \bfOmega_1(b) \opconc \Omega_2)} \in_a \LSInt{A_2}{T}$.
\end{tabular}

\begin{remark}
Notice that the latent interpretation ``takes in'' a computable worldline as an input, therefore 
concretely characterizing the ``latent-ness'' of the definition. The interpretation concerns the 
behavior of a configuration over a period of time. The visible interpretation, on the other the hand
produces worldlines as part of their output (the existential is in the conclusion). This is because 
they describe what new trajectory the configuration would be put on, if interacted by an outside 
entity.
\end{remark}

A few facts can be proved for above definition

\begin{lemma}
The logical relations defined respects the equivalence between computable worldlines: 
\begin{itemize}
  \item If $\gl{w}{\Omega} \in_a \LInt{A}{T}$ and $\cwlequiv{w}{w'}$ then $\gl{w'}{\Omega} \in_a \LInt{A}{T}$.
  \item If $\gl{w}{\Omega} \in_a \LSInt{A}{T}$ and $\cwlequiv{w}{w'}$ then $\gl{w'}{\Omega} \in_a \LSInt{A}{T}$.
\end{itemize}
\end{lemma}

\begin{proof}
Should be straightforward from the definitions.
\end{proof}

\begin{theorem}
If $\gl{w}{\Omega} \in_a \LInt{A}{T}$ and $\IsOf{s}{\cwls{T'}{T}{\Omega'}{\Omega}}$,
then $\gl{(\concat{s}{w})}{\Omega'} \in_a \LInt{A}{T'}$
\end{theorem}
\begin{proof}
Our goal is to show that for all $\IsOf{t}{c}$, $t \geq T'$ and that
$(\concat{s}{w})(t) \in_a \LInt{\expose{A}{t}}{T'}$. 
We know for all $\IsOf{t}{c}$, $t \geq T$ and $w(t) \in_a \LInt{\expose{A}{t}}{T'}$. 
From existence of $s$ we know $T \geq T'$ therefore $t \geq T \geq T'$. 
We know $\cwlequivt{\TIntInf{T}}{\concat{s}{w}}{w}$, therefore we compute $(\concat{s}{w})(t) = w(t)$, 
this concludes what we want to show.
\end{proof}

\begin{theorem}[Forward closure]
If $\gl{w}{\Omega} \in_a \LSInt{A}{T}$ then $\forall\, t \in \TIntInf{T}$, $\gl{(\cutoff{w}{t})}{w(t)} \in_a \LSInt{A}{t}$
\end{theorem}
\begin{proof}
Fix $t$. Our goal is to show that for all $\IsOf{t'}{c}$ and $t' \geq T'$, 
$(\cutoff{w}{t})(t') \in \VInt{\expose{A}{t'}}{t'}$.  Fix $t'$.
We know for all $\IsOf{t'}{c}$ and $t' \geq T$, $w(t') \in \VInt{\expose{A}{t'}}{t'}$.
Since $t' \geq T'$ and $T' \geq T$ therefore $t' \geq T$. On the other hand, $(\cutoff{w}{t})(t') = w(t)$.
This concludes our proof.
\end{proof}

\begin{theorem}[Forward Retyping]
If $\gl{w}{\Omega} \in_a \LSInt{A^c}{T}$ and $\FwdComp{A^c}{B^d}{T}$ then $\gl{w}{\Omega} \in_a \LInt{B^d}{T}$.
\end{theorem}
\begin{proof}
Proof proceeds by induction over structure of $A$. 

In every case, we need to show that:
for all $\IsOf{t}{d}$, $t \in \TIntInf{T}$ and $w(t) \in_a \VInt{\expose{A'}{t}}{t}$.

Invert $\FwdComp{A^c}{B^d}{T}$. Find $\IsOf{t}{d} \entails{\IsOf{t}{\landcst{(\cgeqcst{T})}{c}}}$.

From assumption $\IsOf{t}{d}$, conclude $t \in \TIntInf{T}$ and $\IsOf{t}{c}$.

From assumption, we have for all $\IsOf{t}{c}$ and $t \in \TIntInf{T}$ and $w(t) \in_a \VSInt{\expose{A^c}{t}}{t}$.

What remains is to conclude $w(t) \in_a \VInt{\expose{B^d}{t}}{t}$, which we have to examine each case individually.

\begin{itemize}
  \item \textsc{Case $A^c = \tpunitstycst{t}{p}$.} 

  From inversion we have $B^d = \tpunitstycst{t}{d}$. Notice that $\expose{A^c}{t} = \unitstycst = \expose{B^d}{t}$.

  Therefore $w(t) \in_a \VSInt{\expose{A^c}{t}}{t}$ is just $w(t) \in_a \VSInt{\expose{B^d}{t}}{t}$.

  By definition $\VSInt{\unitstycst}{t}$ and $\VInt{\unitstycst}{t}$ coincide. 

  We therefore conclude what we want to show.

  \item \textsc{Case $A^c = \tptensorstycst{t}{c}{A_1}{A_2}$.}

  From inversion we have $B^d = \tptensorstycst{t}{d}{B_1}{B_2}$ with: 
  
  \begin{itemize}
    \item $\IsOf{t}{d} \entails{\FwdComp{A_1}{B_1}{t}}$, and 
    \item $\IsOf{t}{d} \entails{\FwdComp{A_2}{B_2}{t}}$.
  \end{itemize}

  For the $t$ chosen, by substitution conclude $\FwdComp{A_1}{B_1}{t}$ and $\FwdComp{A_2}{B_2}{t}$.

  From assumption we know there exists $\Omega_1$, $\Omega_2$:
  \begin{itemize}
    \item Exists $w_1$ s.t. $\gl{w_1}{(\RunProc{a}{P_2}, \Omega_2)} \in_a \LSInt{A_2}{t}$, and
    \item $\forall b$, exists $w_2$ such that $\gl{w_2}{(\RunProc{b}{P_1}, \Omega_1)} \in_b \LSInt{A_1}{t}$.
    \item $w(t) = \RunProc{a}{\tptensorsndcst{c'}{t}{P_1}{P_2}}, \Omega_1, \Omega_2$
  \end{itemize}

  By induction conclude 
  \begin{itemize}
    \item Exists $w_1$ s.t. $\gl{w_1}{(\RunProc{a}{P_2}, \Omega_2)} \in_a \LInt{B_2}{t}$, and
    \item $\forall b$, exists $w_2$ such that $\gl{w_2}{(\RunProc{b}{P_1}, \Omega_1)} \in_b \LInt{B_1}{t}$.
  \end{itemize}

  Therefore, by definition conclude $w(t) \in_a \VInt{B^d}{t}$

  \item \textsc{Case $A^c = \tplarrstycst{t}{c}{A_1}{A_2}$.}

  From inversion we have $B^d = \tplarrstycst{t}{d}{B_1}{B_2}$ with: 
  
  \begin{itemize}
    \item $\IsOf{t}{d} \entails{\FwdComp{B_1}{A_1}{t}}$, and 
    \item $\IsOf{t}{d} \entails{\FwdComp{A_2}{B_2}{t}}$.
  \end{itemize}

  For the $t$ chosen, by substitution conclude $\FwdComp{B_1}{A_1}{t}$ and $\FwdComp{A_2}{B_2}{t}$.
  
  From assumption we know there exists $\Omega_2$: 
  \begin{itemize}
    \item $\forall_b$ and $\forall\, \gl{w_1}{\Omega_1} \in_b \LInt{A_1}{t}$,
          $\exists w_2$, $\gl{w_2}{(\RunProc{a}{\Subst{b}{x}{P}}, \Omega_1, \Omega_2)} \in_a \LSInt{A_2}{t}$.
    \item $w(t) = \RunProc{a}{\tplarrrcvcst{c}{t}{x}{P}}, \Omega_2$ 
  \end{itemize}

  We want to show that there exists $\Omega_2$:
  \begin{itemize}
    \item $\forall_b$ and $\forall\, \gl{w_1}{\Omega_1} \in_b \LSInt{B_1}{t}$, 
          $\exists w_2$, $\gl{w_2}{(\RunProc{a}{\Subst{b}{x}{P}}, \Omega_1, \Omega_2)} \in_a \LInt{B_2}{t}$.
    \item $w(t) = \RunProc{a}{\tplarrrcvcst{c}{t}{x}{P}}, \Omega_2$
  \end{itemize}

  Take $\Omega_2$ as the one supplied from the assumption. 

  Fix channel $b$ and $\gl{w_1}{\Omega_1} \in_b \LSInt{A_1}{t}$ from the proof obligation.

  Our goal now is to show there exists $w_2$ 
  s.t. $\gl{w_2}{(\RunProc{a}{\Subst{b}{x}{P}}, \Omega_1, \Omega_2)} \in_a \LInt{B_2}{t}$.

  By induction $\gl{w_1}{\Omega_1} \in_b \LInt{A_1}{t}$.

  Therefore, by assumption conclude there exists $w_2$, 
  $\gl{w_2}{(\RunProc{a}{\Subst{b}{x}{P}}, \Omega_1, \Omega_2)} \in_a \LSInt{A_2}{t}$.

  Take this $w_2$ for the proof goal. By induction conclude what we want to show.

  \item \textsc{Case $A^c = \tpwithstycst{t}{c}{A_1}{A_2}$}

  From inversion we have $B^d = \tptensorstycst{t}{d}{B_1}{B_2}$ with: 
  
  \begin{itemize}
    \item $\IsOf{t}{d} \entails{\FwdComp{A_1}{B_1}{t}}$, and 
    \item $\IsOf{t}{d} \entails{\FwdComp{A_2}{B_2}{t}}$.
  \end{itemize}

  For the $t$ chosen, by substitution conclude $\FwdComp{A_1}{B_1}{t}$ and $\FwdComp{A_2}{B_2}{t}$.

  From assumption we know there exists $\Omega'$ such that:
  \begin{itemize}
    \item $\exists{w_1}$ s.t. $\gl{w_1}{(\RunProc{a}{P_1}, \Omega')} \in_a \LSInt{A_1}{t}$, and  
    \item $\exists{w_2}$ s.t. $\gl{w_2}{(\RunProc{a}{P_2}, \Omega')} \in_a \LSInt{A_2}{t}$.
    \item $w(t) = \RunProc{a}{\tpoffercst{c}{t}{P_1}{P_2}}, \Omega'$,  
  \end{itemize}

  We are to show that for some $\Omega'$:
  \begin{itemize}
    \item $\exists{w_1}$ s.t. $\gl{w_1}{(\RunProc{a}{P_1}, \Omega')} \in_a \LInt{B_1}{t}$, and  
    \item $\exists{w_2}$ s.t. $\gl{w_2}{(\RunProc{a}{P_2}, \Omega')} \in_a \LInt{B_2}{t}$.
    \item $w(t) = \RunProc{a}{\tpoffercst{c}{t}{P_1}{P_2}}, \Omega'$,  
  \end{itemize}

  Fix $w_1$, $w_2$, and $\Omega'$ as supplied by the assumption. 

  Conclude what we want to show by induction.

  \item \textsc{Case $A^c = \tpsumstycst{t}{c}{A_1}{A_2}$.}

  From inversion we have $B^d = \tptensorstycst{t}{d}{B_1}{B_2}$ with: 
  
  \begin{itemize}
    \item $\IsOf{t}{d} \entails{\FwdComp{A_1}{B_1}{t}}$, and 
    \item $\IsOf{t}{d} \entails{\FwdComp{A_2}{B_2}{t}}$.
  \end{itemize}

  For the $t$ chosen, by substitution conclude $\FwdComp{A_1}{B_1}{t}$ and $\FwdComp{A_2}{B_2}{t}$.

  From assumption we know either 
  \begin{itemize}
    \item $w(t) = \RunProc{a}{\tpinlcst{c}{t}{A_1}{A_2}{P}}, \Omega'$ and 
          $\exists w$ s.t. $\gl{w}{(\RunProc{a}{P}, \Omega')} \in_a \LSInt{A_1}{t}$, or  
    \item $w(t) = \RunProc{a}{\tpinrcst{c}{t}{A_1}{A_2}{P}}, \Omega'$ and 
          $\exists w$ s.t. $\gl{w}{(\RunProc{a}{P}, \Omega') \in_a \LSInt{A_2}{t}}$.
  \end{itemize}

  We are to show that either 
  \begin{itemize}
    \item $w(t) = \RunProc{a}{\tpinlcst{c}{t}{A_1}{A_2}{P}}, \Omega'$ and 
          $\exists w$ s.t. $\gl{w}{(\RunProc{a}{P}, \Omega')} \in_a \LInt{B_1}{t}$, or  
    \item $w(t) = \RunProc{a}{\tpinrcst{c}{t}{A_1}{A_2}{P}}, \Omega'$ and 
          $\exists w$ s.t. $\gl{w}{(\RunProc{a}{P}, \Omega') \in_a \LInt{B_2}{t}}$.
  \end{itemize}

  Case analyze our assumption. 
  
  In either case take $\Omega'$ and $w$ as the one supplied from the assumption, 
  then appeal to the IH.
\end{itemize}
We have considered all cases.
\end{proof}

\begin{theorem}[Cut Retyping]
If $\gl{w}{\Omega} \in_a \LInt{A^c}{T}$ and $\CutComp{A^c}{B^d}{T}$ then 
$\gl{w}{\Omega} \in_a \LSInt{B^d}{T}$.
\end{theorem}
\begin{proof}
Proof proceeds by induction over structure of $A$. 

In every case, we need to show that:
for all $\IsOf{t}{d}$ and $t \in \TIntInf{T}$, $w(t) \in_a \VSInt{\expose{A'}{t}}{t}$.

Invert $\CutComp{A^c}{B^d}{T}$. 
Find $\IsOf{t}{\clandcst{(\cgeqcst{T})}{d}} \entails{\IsOf{t}{c}}$.

From assumption conclude $\IsOf{t}{c}$.

Also from assumptions, we have for all $\IsOf{t}{c}$,  $t \in \TIntInf{T}$ and $w(t) \in_a \VInt{\expose{A^c}{t}}{t}$.

What remains is to conclude $w(t) \in_a \VSInt{\expose{B^d}{t}}{t}$, which we have to examine each case individually.

\begin{itemize}
  \item \textsc{Case $A^c = \tpunitstycst{t}{p}$.} 

  From inversion we have $B^d = \tpunitstycst{t}{d}$. Notice that $\expose{A^c}{t} = \unitstycst = \expose{B^d}{t}$.

  Therefore $w(t) \in_a \VInt{\expose{A^c}{t}}{t}$ is just $w(t) \in_a \VInt{\expose{B^d}{t}}{t}$.

  By definition $\VInt{\unitstycst}{t}$ and $\VSInt{\unitstycst}{t}$ coincide. 

  We therefore conclude what we want to show.

  \item \textsc{Case $A^c = \tptensorstycst{t}{c}{A_1}{A_2}$.}

  From inversion we have $B^d = \tptensorstycst{t}{d}{B_1}{B_2}$ with: 
  
  \begin{itemize}
    \item $\IsOf{t}{\landcst{(\cgeqcst{T})}{d}} \entails{\CutComp{A_1}{B_1}{t}}$, and 
    \item $\IsOf{t}{\landcst{(\cgeqcst{T})}{d}} \entails{\CutComp{A_2}{B_2}{t}}$.
  \end{itemize}

  For the $t$ chosen, by substitution conclude $\CutComp{A_1}{B_1}{t}$ and $\CutComp{A_2}{B_2}{t}$.

  From assumption we know there exists $\Omega_1$, $\Omega_2$:
  \begin{itemize}
    \item Exists $w_1$ s.t. $\gl{w_1}{(\RunProc{a}{P_2}, \Omega_2)} \in_a \LSInt{A_2}{t}$, and
    \item $\forall b$, exists $w_2$ such that $\gl{w_2}{(\RunProc{b}{P_1}, \Omega_1)} \in_b \LSInt{A_1}{t}$.
    \item $w(t) = \RunProc{a}{\tptensorsndcst{c'}{t}{P_1}{P_2}}, \Omega_1, \Omega_2$
  \end{itemize}

  By induction conclude 
  \begin{itemize}
    \item Exists $w_1$ s.t. $\gl{w_1}{(\RunProc{a}{P_2}, \Omega_2)} \in_a \LInt{B_2}{t}$, and
    \item $\forall b$, exists $w_2$ such that $\gl{w_2}{(\RunProc{b}{P_1}, \Omega_1)} \in_b \LInt{B_1}{t}$.
  \end{itemize}

  Therefore, by definition conclude $w(t) \in_a \VInt{B^d}{t}$

  \item \textsc{Case $A^c = \tplarrstycst{t}{c}{A_1}{A_2}$.}

  From inversion we have $B^d = \tplarrstycst{t}{d}{B_1}{B_2}$ with: 
  
  \begin{itemize}
    \item $\IsOf{t}{\landcst{(\cgeqcst{T})}{d}} \entails{\FwdComp{B_1}{A_1}{t}}$, and 
    \item $\IsOf{t}{\landcst{(\cgeqcst{T})}{d}} \entails{\CutComp{A_2}{B_2}{t}}$.
  \end{itemize}

  For the $t$ chosen, by substitution conclude $\CutComp{B_1}{A_1}{t}$ and $\CutComp{A_2}{B_2}{t}$.
  
  From assumption we know there exists $\Omega_2$: 
  \begin{itemize}
    \item $\forall_b$ and $\forall\, \gl{w_1}{\Omega_1} \in_b \LInt{A_1}{t}$,
          $\exists w_2$, $\gl{w_2}{(\RunProc{a}{\Subst{b}{x}{P}}, \Omega_1, \Omega_2)} \in_a \LSInt{A_2}{t}$.
    \item $w(t) = \RunProc{a}{\tplarrrcvcst{c}{t}{x}{P}}, \Omega_2$ 
  \end{itemize}

  We want to show that there exists $\Omega_2$:
  \begin{itemize}
    \item $\forall_b$ and $\forall\, \gl{w_1}{\Omega_1} \in_b \LSInt{B_1}{t}$, 
          $\exists w_2$, $\gl{w_2}{(\RunProc{a}{\Subst{b}{x}{P}}, \Omega_1, \Omega_2)} \in_a \LInt{B_2}{t}$.
    \item $w(t) = \RunProc{a}{\tplarrrcvcst{c}{t}{x}{P}}, \Omega_2$
  \end{itemize}

  Take $\Omega_2$ as the one supplied from the assumption. 

  Fix channel $b$ and $\gl{w_1}{\Omega_1} \in_b \LSInt{A_1}{t}$ from the proof obligation.

  Our goal now is to show there exists $w_2$ 
  s.t. $\gl{w_2}{(\RunProc{a}{\Subst{b}{x}{P}}, \Omega_1, \Omega_2)} \in_a \LInt{B_2}{t}$.

  By induction $\gl{w_1}{\Omega_1} \in_b \LInt{A_1}{t}$.

  Therefore, by assumption conclude there exists $w_2$, 
  $\gl{w_2}{(\RunProc{a}{\Subst{b}{x}{P}}, \Omega_1, \Omega_2)} \in_a \LSInt{A_2}{t}$.

  Take this $w_2$ for the proof goal. By induction conclude what we want to show.

  \item \textsc{Case $A^c = \tpwithstycst{t}{c}{A_1}{A_2}$}

  From inversion we have $B^d = \tptensorstycst{t}{d}{B_1}{B_2}$ with: 
  
  \begin{itemize}
    \item $\IsOf{t}{\landcst{(\cgeqcst{T})}{d}} \entails{\CutComp{A_1}{B_1}{t}}$, and 
    \item $\IsOf{t}{\landcst{(\cgeqcst{T})}{d}} \entails{\CutComp{A_2}{B_2}{t}}$.
  \end{itemize}

  For the $t$ chosen, by substitution conclude $\CutComp{A_1}{B_1}{t}$ and $\CutComp{A_2}{B_2}{t}$.

  From assumption we know there exists $\Omega'$ such that:
  \begin{itemize}
    \item $\exists{w_1}$ s.t. $\gl{w_1}{(\RunProc{a}{P_1}, \Omega')} \in_a \LSInt{A_1}{t}$, and  
    \item $\exists{w_2}$ s.t. $\gl{w_2}{(\RunProc{a}{P_2}, \Omega')} \in_a \LSInt{A_2}{t}$.
    \item $w(t) = \RunProc{a}{\tpoffercst{c}{t}{P_1}{P_2}}, \Omega'$,  
  \end{itemize}

  We are to show that for some $\Omega'$:
  \begin{itemize}
    \item $\exists{w_1}$ s.t. $\gl{w_1}{(\RunProc{a}{P_1}, \Omega')} \in_a \LInt{B_1}{t}$, and  
    \item $\exists{w_2}$ s.t. $\gl{w_2}{(\RunProc{a}{P_2}, \Omega')} \in_a \LInt{B_2}{t}$.
    \item $w(t) = \RunProc{a}{\tpoffercst{c}{t}{P_1}{P_2}}, \Omega'$,  
  \end{itemize}

  Fix $w_1$, $w_2$, and $\Omega'$ as supplied by the assumption. 

  Conclude what we want to show by induction.

  \item \textsc{Case $A^c = \tpsumstycst{t}{c}{A_1}{A_2}$.}

  From inversion we have $B^d = \tptensorstycst{t}{d}{B_1}{B_2}$ with: 
  
  \begin{itemize}
    \item $\IsOf{t}{\landcst{(\cgeqcst{T})}{d}} \entails{\CutComp{A_1}{B_1}{t}}$, and 
    \item $\IsOf{t}{\landcst{(\cgeqcst{T})}{d}} \entails{\CutComp{A_2}{B_2}{t}}$.
  \end{itemize}

  For the $t$ chosen, by substitution conclude $\CutComp{A_1}{B_1}{t}$ and $\CutComp{A_2}{B_2}{t}$.

  From assumption we know either 
  \begin{itemize}
    \item $w(t) = \RunProc{a}{\tpinlcst{c}{t}{A_1}{A_2}{P}}, \Omega'$ and 
          $\exists w$ s.t. $\gl{w}{(\RunProc{a}{P}, \Omega')} \in_a \LSInt{A_1}{t}$, or  
    \item $w(t) = \RunProc{a}{\tpinrcst{c}{t}{A_1}{A_2}{P}}, \Omega'$ and 
          $\exists w$ s.t. $\gl{w}{(\RunProc{a}{P}, \Omega') \in_a \LSInt{A_2}{t}}$.
  \end{itemize}

  We are to show that either 
  \begin{itemize}
    \item $w(t) = \RunProc{a}{\tpinlcst{c}{t}{A_1}{A_2}{P}}, \Omega'$ and 
          $\exists w$ s.t. $\gl{w}{(\RunProc{a}{P}, \Omega')} \in_a \LInt{B_1}{t}$, or  
    \item $w(t) = \RunProc{a}{\tpinrcst{c}{t}{A_1}{A_2}{P}}, \Omega'$ and 
          $\exists w$ s.t. $\gl{w}{(\RunProc{a}{P}, \Omega') \in_a \LInt{B_2}{t}}$.
  \end{itemize}

  Case analyze our assumption. 
  
  In either case take $\Omega'$ and $w$ as the one supplied from the assumption, 
  then appeal to the IH.
\end{itemize}
We have considered all cases.
\end{proof}


\begin{theorem}[FTLR]
If $\calF \mid \Delta \entails{\IsOfProc{P}{A}{T}}$ then $\calF \mid \Delta \sementails{\IsOfProc{P}{A}{T}}$.
\end{theorem}
\begin{proof}
Proof by induction on the typing derivation.

In all following cases, one starts by fixing an arbitrary $\IsOf{\varphi}{\calF}$ and try to 
show 
$ \hat{\Delta} \sementails{\IsOfProc{\hat{P}}{\hat{A}}{\hat{T}}} $

Fix $\gl{w_a}{\Omega_a} \in \LSInt{\hat{\Delta}}{\hat{T}}$, a channel $a$ and to show: 
$\exists w$ s.t. $\gl{w}{\conc{(\concfam{a \in \hatDelta}{\Omega_a})}{\RunProc{a}{\hat{P}}}} \in_a \LInt{\hat{A}^{\hat{c}}}{\hat{T}}$.


Now we preform the case analysis: 

\begin{itemize}
  \item \textsc{Case $P = \tpfwdcst{T}{x}$}

    In this case $\hatDelta = \IsOf{x}{A'}$ and we have $\calF \entails{\FwdComp{A'}{A}{T}}$. 
    That is $\FwdComp{\hatA'}{\hatA}{\hatT}$.

    By forward retyping lemma we conclude 
    $\gl{w_x}{\Omega_x} \in_x \LInt{\hatA}{\hatT}$. 

    Rename $x$ in $\Omega_x$ to $a$, and there exists $\gl{w_a}{\Omega_a} \in_x \LInt{\hatA}{\hatT}$. 

    By dynamics $\conc{\Omega_x}{\RunProc{a}{\tpfwdcst{\hatT}{x}}} \UStepsTo{\hatT} \Omega_a$. 

    Therefore conclude by backwards closure.

  \item \textsc{Case $P = \tpspawnproccst{T}{P}{x}{Q}$}

    In this case $\hatDelta = \hatDelta_1, \hatDelta_2$ and we have $\calF \entails{\CutComp{A}{B}{T}}$.

    Induction hypothesis: 

    \begin{enumerate}
      \item $\calF \mid \Delta_1 \sementails{\IsOfProc{P}{T}{A}}$
      \item $\calF \mid \Delta_2, \IsOf{x}{B} \sementails{\IsOfProc{Q}{T}{C}}$
    \end{enumerate}

    Instantiate IH1 to find exists $w_1$ s.t.
    $\gl{w_1}{\conc{(\concfam{a \in \Delta_1}{\Omega_a})}{\RunProc{a}{\hatP}}} \in_a \LInt{\hatA}{\hatT}$

    By cut retyping lemma, conclude $\gl{w_1}{\conc{(\concfam{b \in \Delta_1})}{\RunProc{b}{\hatP}}} \in_b \LSInt{\hatB}{\hatT}$

    Take $w_a$ for $a \in \Delta_2$ and $w_1$ and instantiate IH2, conclude that there exists $w$ s.t. 

    $\gl{w}{
      (\concfam{a \in \Delta_2}{\Omega_a}) \opconc
      ((\concfam{a \in \Delta_1}{\Omega_a}) \opconc \RunProc{b}{\hatP}) \opconc
      \RunProc{a}{\Subst{b}{x}{\hatQ}}
      } \in_a \LInt{\hatC}{\hatT}$

    Remark that $(\concfam{a \in \Delta_2}{\Omega_a}) \opconc ((\concfam{a \in \Delta_1}{\Omega_a})) = (\concfam{a \in \Delta}{\Omega_a})$.

    Therefore $\gl{w}{ (\concfam{a \in \Delta}{\Omega_a}) \opconc \RunProc{b}{\hatP} \opconc \RunProc{a}{\Subst{b}{x}{\hatQ}} } \in_a \LInt{\hatC}{\hatT}$

    Since by dynamics:

    $\conc{(\concfam{a \in \Delta}{\Omega_a})}{\RunProc{a}{\tpspawnproccst{\hatT}{P}{x}{Q}}} 
      \UStepsTo{\hatT}  
    (\concfam{a \in \Delta}{\Omega_a}) \opconc \RunProc{b}{\hatP} \opconc \RunProc{a}{\Subst{b}{x}{\hatQ}}$

    Conclude what we want to show by backwards closure.

  \item \textsc{Case $P = \tpclosecst{t}{p}$}

    In this case $\hatDelta$ is empty.

    Set $w \triangleq \constcwl{\hatT}{\RunProc{a}{\tpclosecst{\hatc}}}$

    To show: for all $\IsOf{t}{\hatc}$, $t \geq \hatT$ and $w(t) \in_a \VInt{\expose{\tpunitstycst{t}{\hatc}}{t}}{t}$.

    Compute $w(t) = (\constcwl{\hatT}{\RunProc{a}{\tpclosecst{\hatc}}})(t) = \RunProc{a}{\tpclosecst{\hatc}}$.

    By definition we have what we want to show.

  \item \textsc{Case $P = \tpwaitcst{T}{x}{Q}$}

    In this case the context is $\Delta, \IsOf{x}{\tpunitstycst{t}{c}}$

    Let $s_a$ be the witnesses of cutoffs $\cutoff{w_a}{\hatT'}$. In particular, $s_x \in \cwls{\hatT}{\hatT'}{\Omega_x}{w_x(\hatT')}$.

    Since $\gl{w_x}{\Omega_x} \in_x \LSInt{\tpunitstycst{t}{\hatc}}{\hatT}$, and $\IsOf{\hatT'}{\hatc}$, 
    therefore $w_x(\hatT') \in_x \VSInt{\expose{\tpunitstycst{t}{\hatc}}{\hatT'}}{\hatT'}$.

    By definition that is $w_x(\hatT') = \RunProc{x}{\tpclosecst{d}}$ for some $d$ s.t. $\IsOf{\hatT'}{d}$. That is $s_x \in \cwls{\hatT}{\hatT'}{\Omega_x}{\RunProc{x}{\tpclosecst{d}}}$.

    By dynamics $\conc{\RunProc{x}{\tpclosecst{d}}}{\tpwaitcst{\hatT'}{x}{\hatQ}} \UStepsTo{\hatT'} \RunProc{a}{\hatQ}$:

    Therefore, exists $s' \in \cwls{\hatT}{\hatT'}{\conc{\Omega_x}{\tpwaitcst{\hatT'}{x}{\hatQ}}}{\RunProc{a}{\hatQ}}$.

    Therefore $\il{(\ilfam{a \in \hatDelta}{s_a})}{s'} \in \cwls{\hatT}{\hatT'}{\conc{(\concfam{a \in \hatDelta}{\Omega_a})}{\conc{\Omega_x}{\tpwaitcst{\hatT'}{x}{\hatQ}}}}{\conc{(\concfam{a \in \hatDelta}{w_a(\hatT')})}{\RunProc{a}{\hatQ}}}$.

    On the other hand, by IH we have: $\calF \mid \Delta \sementails{\IsOfProc{Q}{T}{C}}$. Thererfore $\hatDelta \sementails{\IsOfProc{\hatQ}{\hatT}{\hatC}}$.

    By forward closure, $\gl{\cutoff{w_a}{\hatT'}}{w_a(\hatT')} \in \LSInt{\hatDelta}{\hatT'}$.

    Therefore further apply IH, there exists $\gl{w}{\conc{(\concfam{a \in \hatDelta}{w_a(T')})}{\RunProc{a}{\hatQ}}} \in_a \LSInt{\hatC}{\hatT'}$

    Conclude what we want to show by backwards closure.

  \item \textsc{Case $P = \tptensorsndcst{c}{t}{P_1}{P_2}$}.
  \begin{itemize}
    \item To show: 
    $\conc{(\concfam{a \in \Delta}{\Omega_a})}{\RunProc{a}{\tptensorsndcst{\hat{c}}{t}{\hat{P}_1}{\hat{P}_2}}}  \in_a \LInt{\tptensorstycst{t}{\hat{c}}{\hat{A}_1}{\hat{A}_2}}{\hat{T}}$
    % \item We know $\Omega \in \LSInt{\Delta_1, \Delta_2}{\hat{T}}$. 
    % \item Therefore exists $\Omega = \Omega_1, \Omega_2$ that 
    %   $\Omega_1 \in \LSInt{\hat{\Delta}_1}{\hat{T}}$ and $\Omega_2 \in \LSInt{\hat{\Delta}_2}{\hat{T}}$.

   \item Pick $w \triangleq \il{(\ilfam{a \in \Delta}{w_a})}{\constcwl{t}{\RunProc{a}{\tptensorsndcst{\hat{c}}{t}{\hat{P}_1}{\hat{P}_2}}}}$

   \item To show: for all $\IsOf{T'}{c}$ then $\IsOf{T'}{\cgeqcst{T}}$ and $w(T') \in_a \VInt{\tensorstycst{\Subst{T'}{t}{A_1}}{\Subst{T'}{t}{A_2}}}{t}$.
   
   \item Fix $\IsOf{T'}{c}$. From premise we also conclude $\IsOf{\hat{T}}{\cleqcst{T'}}$.

   \item Our goal is to show $w(T') \in_a \VInt{\tensorstycst{\Subst{T'}{t}{A_1}}{\Subst{T'}{t}{A_2}}}{T'}$, that is: 

      Exists $\Omega_1'$, $\Omega_2'$ such that $w(T') = \RunProc{a}{\tptensorsndcst{\hat{c}}{t}{\hat{P}_1}{\hat{P}_2}}, \Omega_1', \Omega_2'$, and

      \begin{itemize}
        \item $\exists w_1$, $\gl{w_1}{\RunProc{a}{\Subst{T'}{t}{\hat{P}_2}}}, \Omega'_2 \in_a \LInt{\Subst{T'}{t}{\hat{A}_2}}{T'}$.
        \item For all $b$, $\exists w_2$, $\gl{w_2}{\RunProc{b}{\Subst{T'}{t}{\hat{P}_1}}}, \Omega'_1 \in_b \LInt{\Subst{T'}{t}{\hat{A}_1}}{T'}$.
      \end{itemize}

    \item Let $u \triangleq \ilfam{a \in \Delta_1}{w_a}$ and $v \triangleq \ilfam{a \in \Delta_2}{w_a}$.
      Take $\Omega_1' = u(T')$ and $\Omega_2' = v(T')$.

    \item Notice that by associativity $\cwlequiv{\ilfam{a \in \hatDelta}{w_a}}{\il{(\ilfam{a \in \hatDelta_1}{w_a})}{(\ilfam{a \in \hatDelta_2}{w_a})}} = \il{u}{v}$.

    Hence by congurence $\cwlequiv{w}{\il{\il{u}{v}}{\constcwl{t}{\RunProc{a}{\tptensorsndcst{\hat{c}}{t}{\hat{P}_1}{\hat{P}_2}}}}}$
    
    % Therefore $w(T') = u(T'), v(T'), \RunProc{a}{\tptensorsndcst{\hat{c}}{t}{\hat{P}_1}{\hat{P}_2}} = \Omega_1', \Omega_2', \RunProc{a}{\tptensorsndcst{\hat{c}}{t}{\hat{P}_1}{\hat{P}_2}}$.

    Compute $w(T') = u(T'), v(T'), \RunProc{a}{\tptensorsndcst{\hat{c}}{t}{\hat{P}_1}{\hat{P}_2}} = \Omega_1', \Omega_2', \RunProc{a}{\tptensorsndcst{\hat{c}}{t}{\hat{P}_1}{\hat{P}_2}}$.

    \item Induction hypothesis: 
        \begin{enumerate} 
          \item $\calF, \IsOf{t}{c} \mid \Delta_1 \sementails{\IsOfProc{P_1}{t}{A_1}}$
          \item $\calF, \IsOf{t}{c} \mid \Delta_2 \sementails{\IsOfProc{P_2}{t}{A_2}}$
        \end{enumerate}

    \item Define $\varphi' \triangleq \varphi{[t \mapsto T']}$.  
          Remark that $\IsOf{\varphi'}{(\calF, \IsOf{t}{\hat{c}})}$.

          Instantiate IHs with $\varphi'$. Note that $t$ is not free in $\Delta_1$ and $\Delta_2$. 

          \begin{enumerate} 
            \item $\hatDelta_1 \sementails{\IsOfProc{\Subst{T'}{t}{\hatP_1}}{T'}{\Subst{T'}{t}{\hatA_1}}}$
            \item $\hatDelta_2 \sementails{\IsOfProc{\Subst{T'}{t}{\hatP_2}}{T'}{\Subst{T'}{t}{\hatA_2}}}$
          \end{enumerate}

    \item Let $w^1_a \triangleq \cutoff{w_a}{T'}$ and $w^2_a \triangleq \cutoff{w_a}{T'}$, 
    indexed over $\hatDelta_1$ and $\hatDelta_2$ respectively. 
  
    \item By forward closure: $\gl{w^1_a}{w^1_a(T')} \in \LSInt{\hatDelta_1}{T'}$
          and $\gl{w^2_a}{w^2_a(T')} \in \LSInt{\hatDelta_2}{T'}$.

          Compute that $\overline{w^1_a(T')} = \overline{w_a(T')} = u(T')$.  Similarly $\overline{w^2_a(T')} = v(T')$.

    \item Apply IH to conclude what we want to show.

    % \item Apply IH to find
    %   \begin{itemize}
    %     \item $\forall a, \Omega_1', \RunProc{a}{\Subst{T'}{t}{\hat{P}_1}} \in_a \LInt{\Subst{T'}{t}{\hat{A}_1}}{T'}$
    %     \item $\forall a, \Omega_2', \RunProc{a}{\Subst{T'}{t}{\hat{P}_2}} \in_a \LInt{\Subst{T'}{t}{\hat{A}_2}}{T'}$
    %   \end{itemize}

    % \item These are what are left to shown
  \end{itemize}

  \item \textsc{Case $P = \tptensorrcvcst{x}{T'}{y}{Q}$}.
    \begin{itemize}
    \item To show: 
      $\overline{\Omega_a}, \RunProc{a}{\tptensorrcvcst{x}{\hatT'}{y}{\hatQ}} \in_a \LInt{\hatC}{\hatT}$

    % \item We know $\Omega \in \LSInt{(\hatDelta, \IsOf{x}{\tptensorstycst{t}{\hatc}{\hatA_1}{\hatA_2}})}{\hat{T}}$. 
    % \item Exists $\Omega = \Omega_0, \Omega_x$ that 
    %   $\Omega_0 \in \LSInt{\hatDelta}{\hatT}$ and $\Omega_x \in_x \LSInt{\tptensorstycst{t}{\hatc}{\hatA_1}{\hatA_2}}{\hatT}$.

    \item From premise we know $\IsOf{\hatT}{\cleqcst{\hatT'}}$ and $\IsOf{\hatT'}{\hatC}$.

    \item Therefore we conclude $w_x(\hatT') \in \VSInt{\expose{\tptensorstycst{t}{\hatc}{\hatA_1}{\hatA_2}}{\hatT'}}{\hatT'}$
    
          That is $w_x(\hatT') = \Omega_1, \Omega_2, \RunProc{x}{\tptensorsndcst{c'}{t}{P_1}{P_2}}$ for some $c'$, $\Omega_1$, $\Omega_2$, $P_1$, $P_2$ that 

          \begin{enumerate}
            \item For all $b$, $\exists w_1$, $\gl{w_1}{\RunProc{b}{\Subst{\hatT'}{t}{P_1}}}, \Omega_1 \in_b \LSInt{\Subst{\hatT'}{t}{\hatA_2}}{\hatT'}$
            \item $\exists w_2$, $\gl{w_2}{\RunProc{x}{\Subst{\hatT'}{t}{P_2}}, \Omega_2} \in_x \LSInt{\Subst{\hatT'}{t}{\hatA_2}}{\hatT'}$
          \end{enumerate}

    \item From IH: 
      $\calF \mid \Delta, \IsOf{x}{\Subst{T'}{t}{A_1}}, \IsOf{y}{\Subst{T'}{t}{A_2}}
            \sementails{\IsOfProc{Q}{T'}{C}}$
    \item Therefore:
      $\hatDelta, \IsOf{x}{\Subst{\hatT'}{t}{\hatA_1}}, \IsOf{y}{\Subst{\hatT'}{t}{\hatA_2}}
              \sementails{\IsOfProc{\hatQ}{\hatT'}{\hatC}}$

    \item We now try to apply the IH: 
          \begin{itemize}
            \item For context $\hatDelta$, simply pick $\cutoff{w_a}{T'}$ and $w_a(T')$ then appeal to forward closure.
            \item For variable $x$, fix a fresh channel $b$ and take $\gl{w_2}{\RunProc{b}{\Subst{\hatT'}{t}{P_1}}, \Omega_1 \in_b \LSInt{\Subst{\hatT'}{t}{\hatA_2}}{\hatT'}}$.
            \item For variable $y$, take $\gl{w_1}{\RunProc{x}{\Subst{\hatT'}{t}{P_2}}, \Omega_2} \in_x \LSInt{\Subst{\hatT'}{t}{\hatA_2}}{\hatT'}$. 
          \end{itemize}

          From these conclude for all $c$, there exists $u$ such that $\gl{u}{(\overline{w_a(T')}, \Omega_x, \Omega_y)} \in_c \LInt{\hatC}{\hatT'}$

    \item We now try to appeal to backwards closure.

          Let $w \triangleq \il{(\ilfam{a \in \hatDelta}{w_a})}{\il{w_x}{\constcwl{\hatT'}{\RunProc{a}{\tptensorrcvcst{x}{\hatT'}{y}{\hatQ}}}}}$

          Let $s$ be the witness of $\cutoff{w}{T'}$.  Therefore:

          $\IsOf{s}{\ClockProc{T}, \overline{\Omega_a}, \Omega_x, \RunProc{a}{\tptensorrcvcst{x}{\hatT'}{y}{\hatQ}} 
          \MultiStepsTo{} \ClockProc{T'}, \overline{w_a(T')}, w_x(T'), \RunProc{a}{\tptensorrcvcst{x}{\hatT'}{y}{\hatQ}}}$

          That is $s$ leads to $\overline{w_a(T')}, \Omega_1, \Omega_2, \RunProc{x}{\tptensorsndcst{c'}{t}{P_1}{P_2}}, \RunProc{a}{\tptensorrcvcst{x}{\hatT'}{y}{\hatQ}}$
    
    \item From dynamics we know 
    $\Omega_1, \Omega_2, \RunProc{x}{\tptensorsndcst{c'}{t}{P_1}{P_2}}, \RunProc{a}{\tptensorrcvcst{x}{\hatT'}{y}{\hatQ}} \UStepsTo{T'} \Omega_x, \Omega_y$

    Therefore, there exists a reduction sequence $s'$ that witness it.
    
     \item Appeal to backwards closure with said sequence to finish the proof.
    
    \end{itemize}

  \item \textsc{Case $P = \tpoffercst{c}{t}{P_1}{P_2}$}

    Set $w \triangleq \il{(\ilfam{a \in \hatDelta}{w_a})}{\constcwl{\hatT}{\RunProc{a}{\tpoffercst{c}{t}{P_1}{P_2}}}}$

    To show: for all $\IsOf{t}{\hatc}$, $t \geq \hatT$ and $w(t) \in_a \VInt{\expose{\tpunitstycst{t}{\hatc}}{t}}{t}$.

    Compute $w(t) = \conc{(\concfam{a \in \hatDelta}{(w_a(t))})}{\RunProc{a}{\tpoffercst{c}{t}{P_1}{P_2}}}$.

    To show (with $\Omega' = \concfam{a \in \hatDelta}{(w_a(t))}$)  
    \begin{itemize}
      \item $\exists{w_1}$ s.t. $\gl{w_1}{(\RunProc{a}{P_1}, \Omega')} \in_a \LAnyInt{\hatA_1}{t}$, and  
      \item $\exists{w_2}$ s.t. $\gl{w_2}{(\RunProc{a}{P_2}, \Omega')} \in_a \LAnyInt{\hatA_2}{t}$.
    \end{itemize}

    From induction: 
    \begin{itemize}
      \item $\calF, \IsOf{t}{c}\mid \Delta \sementails{\IsOfProc{P_1}{t}{A_1}}$
      \item $\calF, \IsOf{t}{c}\mid \Delta \sementails{\IsOfProc{P_2}{t}{A_2}}$
    \end{itemize}

    Threfore by substituting for the temporal variables: 
    \begin{itemize}
      \item $\hatDelta \sementails{\IsOfProc{\hatP_1}{t}{\hatA_1}}$
      \item $\hatDelta \sementails{\IsOfProc{\hatP_2}{t}{\hatA_2}}$
    \end{itemize}

    By forward closure $\gl{\cutoff{w_a}{t}}{w_a(t)} \in \VSInt{\hatDelta}{t}$.

    Threfore
    \begin{itemize}
      \item $\exists w_1$ s.t. $\gl{w_1}{\conc{(\concfam{a \in \hatDelta}{(w_a(t))})}{\RunProc{a}{\hatP_1}}} \in_a \LInt{\hatA_1}{t}$.
      \item $\exists w_2$ s.t. $\gl{w_2}{\conc{(\concfam{a \in \hatDelta}{(w_a(t))})}{\RunProc{a}{\hatP_2}}} \in_a \LInt{\hatA_2}{t}$.
    \end{itemize}

    These are what exactly what we want to show.

  \item \textsc{Cases $P = \tpselectlcst{T}{x}{Q}$ and $P = \tpselectrcst{T}{x}{Q}$}
    
    W.l.o.g. we focus on the left case.

    In this case the context is $\Delta, \IsOf{x}{\tpwithstycst{t}{c}{A_1}{A_2}}$

    Let $s_a$ be the witnesses of cutoffs $\cutoff{w_a}{\hatT'}$. 
    In particular, $s_x \in \cwls{\hatT}{\hatT'}{\Omega_x}{w_x(\hatT')}$.

    Since $\gl{w_x}{\Omega_x} \in_x \LSInt{\tpwithstycst{t}{\hatc}{\hatA_1}{\hatA_2}}{\hatT}$, 
    and $\IsOf{\hatT'}{\hatc}$, 
    therefore $w_x(\hatT') \in_x \VSInt{\expose{\tpwithstycst{t}{\hatc}{\hatA_1}{\hatA_2}}{\hatT'}}{\hatT'}$.

    By definition that is 
    $w_x(\hatT') = \conc{\Omega'}{\RunProc{x}{\tpoffercst{t}{d}{\hatP_1}{\hatP_2}}}$ for some $d$, and that
   
    \begin{itemize}
      \item $\exists{w_1}$ s.t. $\gl{w_1}{\conc{\RunProc{a}{\Subst{\hatT'}{t}{\hatP_1}}}{\Omega'}} \in_a \LAnyInt{\hatA_1}{\hatT'}$, and  
      \item $\exists{w_2}$ s.t. $\gl{w_2}{\conc{\RunProc{a}{\Subst{\hatT'}{t}{\hatP_2}}}{\Omega'}} \in_a \LAnyInt{\hatA_2}{\hatT'}$.
    \end{itemize}

    For the left case, by dynamics:
    $$
    \conc{\conc{\Omega'}{\RunProc{x}{\tpoffercst{t}{d}{\hatP_1}{\hatP_2}}}}{\RunProc{a}{\tpselectrcst{\hatT}{x}{\hatQ}}} 
        \UStepsTo{\hatT'} 
     \conc{\conc{\Omega'}{\RunProc{x}{\Subst{\hatT'}{t}{\hatP_1}}}}{\RunProc{a}{\hatQ}}
     $$

    Therefore, exists 
    $s' \in \cwls{\hatT}{\hatT'}{\conc{\Omega_x}{\RunProc{a}{\tpselectrcst{\hatT}{x}{\hatQ}}}}{\conc{\Omega'}{\RunProc{a}{\hatQ}}}$.

    Therefore 
    $\il{(\ilfam{a \in \hatDelta}{s_a})}{s'} 
    \in \cwls{\hatT}{\hatT'}
      {\conc{(\concfam{a \in \hatDelta}{\Omega_a})}
            {\conc{\Omega_x}{\RunProc{a}{\tpselectrcst{\hatT}{x}{\hatQ}}}}}
      {\conc{(\concfam{a \in \hatDelta}{w_a(\hatT')})}
            {\conc{\conc{\Omega'}{\RunProc{x}{\Subst{\hatT'}{t}{\hatP_1}}}}{\RunProc{a}{\hatQ}}}}$.

    On the other hand, by IH we have: $\calF \mid \Delta, \IsOf{x}{\Subst{T'}{t}{A_1}} \sementails{\IsOfProc{Q}{T}{C}}$. 

    Thererfore $\hatDelta, \IsOf{x}{\Subst{\hatT'}{t}{\hatA_1}} \sementails{\IsOfProc{\hatQ}{\hatT}{\hatC}}$.

    By forward closure, $\gl{\cutoff{w_a}{\hatT'}}{w_a(\hatT')} \in \LSInt{\hatDelta}{\hatT'}$.

    Instantiate the IH together with $w_x \triangleq w_1$, conclude:

    There exists 
    $\gl{w}{\conc{\conc{(\concfam{a \in \hatDelta}{w_a(\hatT')})}{\conc{\RunProc{a}{\Subst{\hatT'}{t}{\hatP_1}}}{\Omega'}}}{\RunProc{a}{\hatQ}}} \in_a \LSInt{\hatC}{\hatT'}$

    Conclude what we want to show by backwards closure.

\item \textsc{Cases $P = \tpinlcst{c}{t}{A_1}{A_2}{P}$ and $P = \tpinrcst{c}{t}{A_1}{A_2}{P}$}

    W.l.o.g. we consider the left injection.

    Set $w \triangleq \il{(\ilfam{a \in \hatDelta}{w_a})}{\constcwl{\hatT}{\RunProc{a}{\tpinlcst{c}{t}{A_1}{A_2}{P}}}}$

    To show: for all $\IsOf{t}{\hatc}$, $t \geq \hatT$ and $w(t) \in_a \VInt{\expose{\tpsumstycst{t}{c}{A_1}{A_2}}{t}}{t}$.

    Compute $w(t) = \conc{(\concfam{a \in \hatDelta}{(w_a(t))})}{\RunProc{a}{\RunProc{a}{\tpinlcst{c}{t}{A_1}{A_2}{P}}}}$.

    To show one of the following (both with $\Omega' = \concfam{a \in \hatDelta}{(w_a(t))}$) :
    \begin{itemize}
      \item $\exists w$ s.t. $\gl{w}{(\RunProc{a}{P}, \Omega')} \in_a \LInt{A_1}{T}$, or  
      \item $\exists w$ s.t. $\gl{w}{(\RunProc{a}{P}, \Omega')} \in_a \LInt{A_2}{T}$.
    \end{itemize}

    For the left injection we will try to establish the left case.

    From induction: $\calF, \IsOf{t}{c}\mid \Delta \sementails{\IsOfProc{P}{t}{A_1}}$.

    Threfore by substituting for the temporal variables: $\hatDelta \sementails{\IsOfProc{\hatP}{t}{\hatA_1}}$

    By forward closure $\gl{\cutoff{w_a}{t}}{w_a(t)} \in \VSInt{\hatDelta}{t}$.

    Threfore
$\exists w$ s.t. $\gl{w}{\conc{(\concfam{a \in \hatDelta}{(w_a(t))})}{\RunProc{a}{\hatP}}} \in_a \LInt{\hatA_1}{t}$.

    This is what exactly what we want to show.

  \item \textsc{Case $P = \tpcasecst{T}{x}{Q_1}{Q_2}$}
    
    In this case the context is $\Delta, \IsOf{x}{\tpsumstycst{t}{c}{A_1}{A_2}}$

    Let $s_a$ be the witnesses of cutoffs $\cutoff{w_a}{\hatT'}$. 
    In particular, $s_x \in \cwls{\hatT}{\hatT'}{\Omega_x}{w_x(\hatT')}$.

    Since $\gl{w_x}{\Omega_x} \in_x \LSInt{\tpsumstycst{t}{\hatc}{\hatA_1}{\hatA_2}}{\hatT}$, 
    and $\IsOf{\hatT'}{\hatc}$, 
    therefore $w_x(\hatT') \in_x \VSInt{\expose{\tpsumstycst{t}{\hatc}{\hatA_1}{\hatA_2}}{\hatT'}}{\hatT'}$.

    By definition that is either 
    \begin{itemize}
      \item $w_x(\hatT') = \conc{\Omega'}{\RunProc{x}{\tpinlcst{t}{d}{A_1}{A_2}{P}}}$, and that
            $\gl{w_1}{\conc{\RunProc{a}{\Subst{\hatT'}{t}{P}}}{\Omega'}} \in_a \LSInt{\hatA_1}{\hatT'}$, or;
      \item $w_x(\hatT') = \conc{\Omega'}{\RunProc{x}{\tpinrcst{t}{d}{A_1}{A_2}{P}}}$, and that
            $\gl{w_2}{\conc{\RunProc{a}{\Subst{\hatT'}{t}{P}}}{\Omega'}} \in_a \LSInt{\hatA_1}{\hatT'}$, or;
    \end{itemize} 

    Focus on the left case (the right case can be treated analogously), by dynamics:
    $$
    \conc{\conc{\Omega'}{\RunProc{x}{\tpinlcst{t}{d}{\hatA_1}{\hatA_2}{\hatP}}}}{\RunProc{a}{\tpcasecst{\hatT'}{x}{\hatQ_1}{\hatQ_2}}} 
        \UStepsTo{\hatT'} 
    \conc{\conc{\Omega'}{\RunProc{x}{\Subst{\hatT'}{t}{\hatP}}}}{\RunProc{a}{\hatQ_1}}
    $$

    Therefore, exists 
    $s' \in \cwls{\hatT}{\hatT'}
        {\conc{\Omega_x}{\RunProc{a}{\tpcasecst{\hatT'}{x}{\hatQ_1}{\hatQ_2}}}}
        {\conc{\conc{\Omega'}{\RunProc{x}{\Subst{\hatT'}{t}{\hatP}}}}{\RunProc{a}{\hatQ_1}}}$.

    Therefore 
    $\il{(\ilfam{a \in \hatDelta}{s_a})}{s'} 
    \in \cwls{\hatT}{\hatT'}
      {\conc{(\concfam{a \in \hatDelta}{\Omega_a})}
            {\conc{\Omega_x}{\RunProc{a}{\tpcasecst{\hatT'}{x}{\hatQ_1}{\hatQ_2}}}}}
      {\conc{(\concfam{a \in \hatDelta}{w_a(\hatT')})}
            {\conc{\conc{\Omega'}{\RunProc{x}{\Subst{\hatT'}{t}{\hatP}}}}{\RunProc{a}{\hatQ}}}}$.

    On the other hand, by IH we have: 
    \begin{itemize}
      \item $\calF \mid \Delta, \IsOf{x}{\Subst{T'}{t}{A_1}} \sementails{\IsOfProc{Q_1}{T}{C}}$. 
      \item $\calF \mid \Delta, \IsOf{x}{\Subst{T'}{t}{A_2}} \sementails{\IsOfProc{Q_2}{T}{C}}$. 
    \end{itemize}

    For the left injection case, we only need the one regarding $A_1$.

    Thererfore $\hatDelta, \IsOf{x}{\Subst{\hatT'}{t}{\hatA_1}} \sementails{\IsOfProc{\hatQ_1}{\hatT}{\hatC}}$.

    By forward closure, $\gl{\cutoff{w_a}{\hatT'}}{w_a(\hatT')} \in \LSInt{\hatDelta}{\hatT'}$.

    Instantiate the IH together with $w_x \triangleq w_1$, conclude:

    There exists 
    $\gl{w}{\conc{\conc{(\concfam{a \in \hatDelta}{w_a(\hatT')})}
                        {\conc{\RunProc{x}{\Subst{\hatT'}{t}{\hatP}}}{\Omega'}}}
                        {\RunProc{a}{\hatQ_1}}} \in_a \LInt{\hatC}{\hatT'}$

    Conclude what we want to show by backwards closure.

  \item \textsc{Cases $P = \tpselectlcst{T}{x}{Q}$ and $P = \tpselectrcst{T}{x}{Q}$}
    
    W.l.o.g. we focus on the left case.

    In this case the context is $\Delta, \IsOf{x}{\tpwithstycst{t}{c}{A_1}{A_2}}$

    Let $s_a$ be the witnesses of cutoffs $\cutoff{w_a}{\hatT'}$. 
    In particular, $s_x \in \cwls{\hatT}{\hatT'}{\Omega_x}{w_x(\hatT')}$.

    Since $\gl{w_x}{\Omega_x} \in_x \LSInt{\tpwithstycst{t}{\hatc}{\hatA_1}{\hatA_2}}{\hatT}$, 
    and $\IsOf{\hatT'}{\hatc}$, 
    therefore $w_x(\hatT') \in_x \VSInt{\expose{\tpwithstycst{t}{\hatc}{\hatA_1}{\hatA_2}}{\hatT'}}{\hatT'}$.

    By definition that is 
    $w_x(\hatT') = \conc{\Omega'}{\RunProc{x}{\tpoffercst{t}{d}{\hatP_1}{\hatP_2}}}$ for some $d$, and that
   
    \begin{itemize}
      \item $\exists{w_1}$ s.t. $\gl{w_1}{\conc{\RunProc{a}{\Subst{\hatT'}{t}{\hatP_1}}}{\Omega'}} \in_a \LAnyInt{\hatA_1}{\hatT'}$, and  
      \item $\exists{w_2}$ s.t. $\gl{w_2}{\conc{\RunProc{a}{\Subst{\hatT'}{t}{\hatP_2}}}{\Omega'}} \in_a \LAnyInt{\hatA_2}{\hatT'}$.
    \end{itemize}

    For the left case, by dynamics:
    $$
    \conc{\conc{\Omega'}{\RunProc{x}{\tpoffercst{t}{d}{\hatP_1}{\hatP_2}}}}{\RunProc{a}{\tpselectrcst{\hatT}{x}{\hatQ}}} 
        \UStepsTo{\hatT'} 
     \conc{\conc{\Omega'}{\RunProc{x}{\Subst{\hatT'}{t}{\hatP_1}}}}{\RunProc{a}{\hatQ}}
     $$

    Therefore, exists 
    $s' \in \cwls{\hatT}{\hatT'}{\conc{\Omega_x}{\RunProc{a}{\tpselectrcst{\hatT}{x}{\hatQ}}}}{\conc{\Omega'}{\RunProc{a}{\hatQ}}}$.

    Therefore 
    $\il{(\ilfam{a \in \hatDelta}{s_a})}{s'} 
    \in \cwls{\hatT}{\hatT'}
      {\conc{(\concfam{a \in \hatDelta}{\Omega_a})}
            {\conc{\Omega_x}{\RunProc{a}{\tpselectrcst{\hatT}{x}{\hatQ}}}}}
      {\conc{(\concfam{a \in \hatDelta}{w_a(\hatT')})}
            {\conc{\conc{\Omega'}{\RunProc{x}{\Subst{\hatT'}{t}{\hatP_1}}}}{\RunProc{a}{\hatQ}}}}$.

    On the other hand, by IH we have: $\calF \mid \Delta, \IsOf{x}{\Subst{T'}{t}{A_1}} \sementails{\IsOfProc{Q}{T}{C}}$. 

    Thererfore $\hatDelta, \IsOf{x}{\Subst{\hatT'}{t}{\hatA_1}} \sementails{\IsOfProc{\hatQ}{\hatT}{\hatC}}$.

    By forward closure, $\gl{\cutoff{w_a}{\hatT'}}{w_a(\hatT')} \in \LSInt{\hatDelta}{\hatT'}$.

    Instantiate the IH together with $w_x \triangleq w_1$, conclude:

    There exists 
    $\gl{w}{\conc{\conc{(\concfam{a \in \hatDelta}{w_a(\hatT')})}{\conc{\RunProc{a}{\Subst{\hatT'}{t}{\hatP_1}}}{\Omega'}}}{\RunProc{a}{\hatQ}}} \in_a \LSInt{\hatC}{\hatT'}$

    Conclude what we want to show by backwards closure.

\item \textsc{Case $P = \tplarrrcvcst{c}{t}{A_1}{x}{P}$}

    Set $w \triangleq \il{(\ilfam{a \in \hatDelta}{w_a})}{\constcwl{\hatT}{\RunProc{a}{\tplarrrcvcst{\hatc}{t}{\hatA_1}{x}{\hatP}}}}$

    To show: for all $\IsOf{t}{\hatc}$, $t \geq \hatT$ and $w(t) \in_a \VInt{\expose{\tplarrstycst{t}{c}{\hatA_1}{\hatA_2}}{t}}{t}$.

    Compute $w(t) = \conc{(\concfam{a \in \hatDelta}{(w_a(t))})}{\RunProc{a}{\RunProc{a}{\tpinlcst{\hatc}{t}{\hatA_1}{\hatA_2}{\hatP}}}}$.

    To show (with $\Omega_2 = \concfam{a \in \hatDelta}{(w_a(t))}$): 

    $\forall b$ and $\forall w_1$ s.t. $\gl{w_1}{\Omega_1} \in_b \LSInt{\hatA_1}{t}$, 
    $\exists w_2$, $\gl{w_2}{\conc{\RunProc{a}{\Subst{b}{x}{\hatP}}}{\conc{\Omega_1}{\Omega_2}}} \in_a \LInt{\hatA_2}{t}$.

    Fix channel $b$, $w_1$ and $\Omega_1$.

    From induction: $\calF, \IsOf{t}{c} \mid \Delta, \IsOf{x}{A_1} \sementails{\IsOfProc{P}{t}{A_2}}$.

    Threfore by substituting for the temporal variables: $\hatDelta, \IsOf{x}{A_2} \sementails{\IsOfProc{\hatP}{t}{\hatA_2}}$

    By forward closure $\gl{\cutoff{w_a}{t}}{w_a(t)} \in \VSInt{\hatDelta}{t}$.

    Together with $w_1$, conclude $\exists w$ s.t. 
    $\gl{w}{\conc{(\concfam{a \in \hatDelta}{(w_a(t))})}{\conc{\Omega_1}{\RunProc{a}{\Subst{b}{x}{\hatP}}}}} \in_a \LInt{\hatA_2}{t}$.

    This is what exactly what we want to show.

  \item \textsc{Case $P = \tplarrsndcst{T'}{x}{P}{Q}$}
    
    In this case the context is $\Delta_1, \Delta_2, \IsOf{x}{\tplarrstycst{t}{c}{A_1}{A_2}}$. Let $\Delta \triangleq \Delta_1, \Delta_2$.

    Let $s_a$ be the witnesses of cutoffs $\cutoff{w_a}{\hatT'}$. 
    In particular, $s_x \in \cwls{\hatT}{\hatT'}{\Omega_x}{w_x(\hatT')}$.

    Since $\gl{w_x}{\Omega_x} \in_x \LSInt{\tplarrstycst{t}{\hatc}{\hatA_1}{\hatA_2}}{\hatT}$, 
    and $\IsOf{\hatT'}{\hatc}$, 
    therefore $w_x(\hatT') \in_x \VSInt{\expose{\tplarrstycst{t}{\hatc}{\hatA_1}{\hatA_2}}{\hatT'}}{\hatT'}$.

    By definition that is $w_x(\hatT') = \RunProc{x}{\tplarrrcvcst{d}{t}{x}{P'}}, \Omega'$ and:

    $\forall_b$ and $\forall\, \gl{w_1}{\Omega_1} \in_b \LInt{\hatA_1}{\hatT'}$,
    $\exists w_2$, $\gl{w_2}{(\RunProc{a}{\Subst{\hatT', b}{t, x}{P'}}, \Omega_1, \Omega')} \in_a \LSInt{\hatA_2}{\hatT'}$.

    From dynamics
    $$
    \conc{\conc{\Omega'}{\RunProc{x}{\tplarrrcvcst{d}{t}{x}{P'}}}}{\RunProc{a}{\tplarrsndcst{\hatT'}{x}{\hatP}{\hatQ}}} 
        \UStepsTo{\hatT'} 
    \conc{\conc{\Omega'}{\conc{\RunProc{x}{\Subst{\hatT', b}{t, x}{P'}}}{\RunProc{b}{\hatP}}}}{\RunProc{a}{\hatQ}}
    $$

    Therefore, exists 
    $s' \in \cwls{\hatT}{\hatT'}
        {\conc{\Omega_x}{\RunProc{a}{\tplarrsndcst{\hatT'}{x}{\hatP}{\hatQ}}}}
        {\conc{\conc{\Omega'}{\conc{\RunProc{x}{\Subst{\hatT', b}{t, x}{P'}}}{\RunProc{b}{\hatP}}}}{\RunProc{a}{\hatQ}}}$.

    Therefore 
    $\il{(\ilfam{a \in \hatDelta}{s_a})}{s'} 
    \in \cwls{\hatT}{\hatT'}
      {\conc{(\concfam{a \in \hatDelta}{\Omega_a})}
            {\conc{\Omega_x}{\RunProc{a}{\tplarrsndcst{\hatT'}{x}{\hatP}{\hatQ}}}}}
      {\conc{(\concfam{a \in \hatDelta}{w_a(\hatT')})}
            {\conc{\conc{\Omega'}{\conc{\RunProc{x}{\Subst{\hatT', b}{t, x}{P'}}}{\RunProc{b}{\hatP}}}}{\RunProc{a}{\hatQ}}}}$.

    On the other hand, by IH we have: 
    \begin{itemize}
      \item $\calF \mid \Delta_1 \sementails{\IsOfProc{P}{T'}{\Subst{T'}{t}{A_1}}}$. 
      \item $\calF \mid \Delta_2, \IsOf{x}{\Subst{T'}{t}{A_2}} \sementails{\IsOfProc{Q}{T'}{C}}$. 
    \end{itemize}

    Thererfore: 
    \begin{itemize}
      \item $\hatDelta_1 \sementails{\IsOfProc{\hatP}{\hatT'}{\Subst{\hatT'}{t}{\hatA_1}}}$.
      \item $\hatDelta_2, \IsOf{x}{\Subst{T'}{t}{\hatA_2}} \sementails{\IsOfProc{\hatQ}{\hatT'}{\hatC}}$. 
    \end{itemize}

    By forward closure, $\gl{\cutoff{w_a}{\hatT'}}{w_a(\hatT')} \in \LSInt{\hatDelta}{\hatT'}$.

    Instantiate the IH1 with $w_a$ with $a \in \Delta_1$ and conclude: 

    There exists $w_1$, s.t. $ \gl{w_1}{\conc{(\concfam{a \in \hatDelta_1}{w_a(\hatT')})}{\RunProc{b}{\hatP}}} \in \LInt{\hatA_1}{\hatT'}$

    Apply the assumption with $w_1$, conclude (with $\Omega_1 = \conc{(\concfam{a \in \hatDelta_1}{w_a(\hatT')})}{\RunProc{b}{\hatP}}$): 
    
    There exists $w_2$ s.t. 
    $\gl{w_2}{(\RunProc{a}{\Subst{\hatT', b}{t, x}{P'}} \opconc \Omega_1 \opconc \Omega')} \in_a \LSInt{\hatA_2}{\hatT'}$.

    Together with $w_a$ for $a \in \Delta_2$, apply IH2 and find there exists $w$ s.t.

    $\gl{w}{ (\concfam{a \in \hatDelta_2}{w_a(\hatT')}) \opconc
              \RunProc{x}{\Subst{\hatT', b}{t, x}{P'}} \opconc \Omega' \opconc
              \conc{(\concfam{a \in \hatDelta_1}{w_a(\hatT')})}{\RunProc{b}{\hatP}} \opconc
              \RunProc{a}{\hatQ}} \in_a \LInt{\hatC}{\hatT'}$

    Remark that $(\concfam{a \in \hatDelta}{w_a(\hatT')}) = \conc{\concfam{a \in \hatDelta_1}{w_a(\hatT')}}{(\concfam{a \in \hatDelta_2}{w_a(\hatT')})}$

    Therefore
    $\gl{w}{(\concfam{a \in \hatDelta}{w_a(\hatT')}) \opconc
             \RunProc{x}{\Subst{\hatT', b}{t, x}{P'}} \opconc \Omega' \opconc
             \RunProc{b}{\hatP} \opconc
             \RunProc{a}{\hatQ}} \in_a \LInt{\hatC}{\hatT'}$

    Conclude what we want to show by backwards closure.
\end{itemize}
\end{proof}

==> contents/temporal.tex <==

\paragraph{Program Syntax} Here are the syntax for the programs


\paragraph{Statics} 
% Judgment $\boxed{\calF \entails{\IsOf{T}{c}}}$ asserts the point in time $T$ satisfies $c$. 
% Judgment $\boxed{\calF \entails{\IsBefore{T}{T'}}}$ asserts the point in time $T$ preceeds $T'$. 

% Judgment $\boxed{\calF \entails{\IsFrame{T}}}$ asserts that $T$ is a valid frame given $\calF$.

% Judgment $\boxed{\calF \entails{\IsFType{c}}}$ asserts that $c$ is a valid condition given $\calF$.

Judgment $\boxed{\calG; \calF \entails{\IsSType{A}}}$ states that $A$ is a \emph{session} type 
assuming points in time in $\calF$. Typing judgments mentioning session types presupposes 
all types are well formed.

Judgment $\boxed{\calG; \calF \mid \Delta \entails{\IsOfProc{P}{T}{A}}}$ asserts that given a context of frames 
of references (i.e. points in time) $\calF$, the process $P$, having access to (tempral) resources in 
$\Delta$, if ``activated'' at time $T$, provides a (temporal) service $A$ at its offering channel.

User programs are always typed with an initial context $\calG_0 \triangleq t_0$ and $\calF$, $\Delta$ both empty at $T = t_0$.

$\boxed{\calG; \calF \entails{\IsSType{A}}}$
\begin{mathpar}
\inferrule[]
{\calG, t; \calF \entails{\IsProp{p}}}
{\calG; \calF \entails{\IsSType{\tpunitstycst{t}{p}}}}

\inferrule[]
{\calG, t; \calF \entails{\IsProp{c}} \\  
 \calG, t; \calF \entails{\IsSType{A_1}} \\ 
 \calG, t; \calF \entails{\IsSType{A_2}} }
{\calG \entails{\IsSType{\tptensorstycst{t}{p}{A_1}{A_2}}}}

\inferrule[]
{\calG, t; \calF \entails{\IsProp{c}} \\  
 \calG, t; \calF \entails{\IsSType{A_1}} \\ 
 \calG, t; \calF \entails{\IsSType{A_2}} }
{\calG; \calF \entails{\IsSType{\tplarrstycst{t}{p}{A_1}{A_2}}}}

\inferrule[]
{\calG, t; \calF \entails{\IsProp{p}} \\  
 \calG, t; \calF \entails{\IsSType{A_1}} \\ 
 \calF, t; \calF \entails{\IsSType{A_2}} }
{\calG; \calF \entails{\IsSType{\tpsumstycst{t}{p}{A_1}{A_2}}}}

\inferrule[]
{\calG, t; \calF \entails{\IsProp{p}} \\  
 \calG, t; \calF \entails{\IsSType{A_1}} \\ 
 \calG, t; \calF \entails{\IsSType{A_2}} }
{\calG; \calF \entails{\IsSType{\tpwithstycst{t}{p}{A_1}{A_2}}}}
\end{mathpar}

$\boxed{\calG; \calF \entails{\IsCtx{\Delta}}}$
\begin{mathpar}
\inferrule
{\strut}
{\calG; \calF \entails{\IsCtx{\emptyset}}}

\inferrule
{\calG; \calF \entails{\IsCtx{\Delta}} \\ 
 \calG; \calF \entails{\IsSType{A}}}
{\calG; \calF \entails{\IsCtx{(\emptyset, \IsOf{x}{A})}}}
\end{mathpar}

% \begin{remark}
% The set of rules looks very similar to ones you would find in a dependently typed 
% language. In particular, the temporal layer strongly resembles that of a functional, 
% dependently typed language. 

% Some caveats: 
% \begin{itemize}
%   \item We need to define a judgment $\boxed{\IsFCtx{\calF}}$ that asserts the well-formedness of the frame context.
%   \item We are missing a judgment that defines well-formedness of durations $\boxed{\calF \entails{\IsDuration{D}}}$.
%   We could elide the definition if we don't allow taking difference of frames (then any syntatically well-formed duration, 
%   is a duration).
% \end{itemize}
% \end{remark}

% It remains to be explained how $\boxed{\calF \entails \TimeIsRight{T}{c}}$ and 
% $\boxed{\calF \entails{\IsBefore{T}{T'}}}$ is decided. Both of the judgments can be reduced 
% to queries in some first order logic, with judgment being 
% $\boxed{\Gamma \mid \calE \entails{Q}}$. 

% That is, given (frame) variables in $\Gamma$, and (temporal) propositions in $P$ in $\calE$, one proves temporal 
% propositions $Q$. The syntax for temporal propositions is as follows:

% \begin{synchart}{tfol}
% \Sort{TProp} & P & \bnfdef & \top          & & \text{Truth} \\
%              &   & \bnfalt & P_1 \land P_2 & & \text{Conjunction} \\
%              &   & \bnfalt & P_1 \lor P_2  & & \text{Disjunction} \\
%              &   & \bnfalt & T_1 = T_2     & & \text{Identity} \\
%              &   & \bnfalt & T_1 \leq T_2  & & \text{No-later} \\
%              &   & \bnfalt & T_1 \geq T_2  & & \text{No-earlier}
% \end{synchart}

% Interpretations into this FOL is intuitive. 

% Conditions are interpreted as \emph{predicates} over frames, defined inductively as follows:
% \begin{align*}
%   \Interp{\ctrivcst}    &\triangleq P(T) \quad\text{iff}\quad  \top \\
%   \Interp{\cequcst{T'}} &\triangleq P(T) \quad\text{iff}\quad  T = T' \\
%   \Interp{\cleqcst{T'}} &\triangleq P(T) \quad\text{iff}\quad T \leq T' \\
%   \Interp{\cgeqcst{T'}} &\triangleq P(T) \quad\text{iff}\quad T \geq T' \\
%   \Interp{\clandcst{c_1}{c_2}} &\triangleq P(T) \quad\text{iff}\quad \Interp{c_1}(T) \land \Interp{c_2}{T}\\
%   \Interp{\clorcst{c_1}{c_2}} &\triangleq P(T) \quad\text{iff}\quad \Interp{c_1}(T) \lor \Interp{c_2}{T}
% \end{align*}

% The dot is interpreted as the argument to the predicate, justifying the notation.

% The context $\calF$ is interpreted as the context of the FOL, defined as follows: 
% \begin{align*}
%   \Interp{\IsOf{t}{c}} &\triangleq t \mid \Interp{c}(t) \\
%   \Interp{\calF, \IsOf{t}{c}} &\triangleq \Gamma, t \mid \calE, \Interp{c}(t) \qquad (\text{assuming $\Interp{\calF} = \Gamma \mid \calE$})
% \end{align*}

% Finally, we are able to specify the interpretations of the judgments: 

% \begin{itemize}
%   \item The judgment $\calF \entails{\TimeIsRight{T}{c}}$ holds iff $\Interp{\calF} \entails{\Interp{c}(T)}$.
%   \item The judgment $\calF \entails{\IsBefore{T_1}{T_2}}$ holds iff $\Interp{\calF} \entails{T_1 \leq T_2}$.
% \end{itemize}

% Now it remains to put down the rules in the FOL. 

% The first move is to define $\geq$ and equality in terms of $\leq$: 

% \begin{mathpar}
% \inferrule[AntiSym]
%   {\Gamma \mid \calE \entails{T \leq T'} \\
%    \Gamma \mid \calE \entails{T' \leq T}}
%   {\Gamma \entails{T = T'}}

% \inferrule[AntiSymInv]
%   {\Gamma \mid \calE \entails{T = T'}}
%   {\Gamma \mid \calE \entails{T \leq T'} \\
%    \Gamma \mid \calE \entails{T' \leq T}} \\

% \inferrule[Geq]
%   {\Gamma \mid \calE \entails{T' \leq T}}
%   {\Gamma \mid \calE \entails{T \geq T'}}

% \inferrule[GeqInv]
%   {\Gamma \mid \calE \entails{T' \geq T}}
%   {\Gamma \mid \calE \entails{T \leq T'}} \\

% \inferrule[Refl]
%   {\strut}
%   {\Gamma \mid \calE \entails{T \leq T}}

% \inferrule[Trans]
%   {\Gamma \mid \calE \entails{T_1 \leq T_2} \\ 
%    \Gamma \mid \calE \entails{T_2 \leq T_3}}
%   {\Gamma \mid \calE \entails{T_1 \leq T_3}}

% \inferrule[Assump]
%   {\strut}
%   {\Gamma \mid \calE, P \entails{P}} \\

% \inferrule[LandR]
%   {\Gamma \mid \calE \entails{P_1} \\ 
%    \Gamma \mid \calE \entails{P_2}}
%   {\Gamma \mid \calE \entails{P_2 \land P_2}}

% \inferrule[LandL]
%   {\Gamma \mid \calE, P_1, P_2 \entails{Q}}
%   {\Gamma \mid \calE, P_1 \land P_2 \entails{Q}} \\

% \inferrule[LorR1]
%   {\Gamma \mid \calE \entails{P_1}}
%   {\Gamma \mid \calE \entails{P_1 \lor P_2}}

% \inferrule[LorR2]
%   {\Gamma \mid \calE \entails{P_1}}
%   {\Gamma \mid \calE \entails{P_1 \lor P_2}}

% \inferrule[LorL]
%   {\Gamma \mid \calE, P_1 \entails{Q} \\ 
%    \Gamma \mid \calE, P_2 \entails{Q}}
%   {\Gamma \mid \calE, P_1 \lor P_2 \entails{Q}}

% \inferrule[Shift]
%   {\Gamma \mid \calE \entails{T_1 \leq T_2} \\ 
%    \Gamma \mid \calE \entails{D_1 \leq D_2}}
%   {\Gamma \mid \calE \entails{\fshiftcst{T_1}{D_1} \leq \fshiftcst{T_2}{D_2}}}
% \end{mathpar}

% Above rules should be sufficient. In the last rule $D_1 \leq D_2$ can be defined in the 
% obvious way if we don't allow users to take differences in frames. Otherwise more rules 
% need to be put in.

% Rules concerning reasoning with shifts (such as associativity, replace equals by equals) 
% should be admissible. In the meantime we could have introduced more connectives in the 
% FOL layer, for example the classical temporal connectives. Of course then the question 
% is whether it is SMT-solvable. The current fragment seems decidable.

% \clearpage

\emph{Retyping} relation $\boxed{\FwdComp{A}{A'}{T}}$ restricts the type that a process can 
forward services in its context as. Dually, the \emph{cut Compatibility} $\boxed{\CutComp{A}{A'}{T}}$ relation relaxes the type that 
a process can be used for in other processes' context. They are both defined (independent of each other) inductively.

%% Rules are available in the main paper
\input{rules/retyping}

Now we can define the typing judgments

%% Rules are available in the main paper
%% \input{rules/typing}

\paragraph{Dynamics} The following dynamics is stated with multiset reduction:

\begin{small}
\input{rules/insta-step.tex}
\end{small}

Given the user program $t_0; \emptyset \mid \emptyset \entails{\IsOfProc{P}{t_0}{A}}$, 
the initial configuration is formed by 

$$\Omega_0 \triangleq \ClockProc{\finitcst}, \RunProc{a}{\Subst{\finitcst}{t_0}{P}}$$




==> contents/time.tex <==
\section{Temporal Logic}

% Following a long tradition we present our logic for reasoning about time as quantifier
% free fragment of 2-sorted \emph{first Order Logic}. The logic has the following two syntactic sorts: 
% a sort for \emph{points in time} and a sort for 
% \emph{durations}, which should be thought of as \emph{differences in time}. 

% The logic axiomitizes a binary \emph{less-than-or-equal} relation along with an 
% equality between elements of both sorts.

% The syntax for the logic is presented in the following chart:

% % \input{charts/tlogic.tex}

% Following the tradition the judgment governing the temporal takes the form $\boxed{\calG; \calF \entails{p}}$, 
% where $G = r, s, t \dots$ is a context of variables in the sort $T$ and $\calF = p_1, \dots, p_n$ is a context of 
% propositions.

% The rules for this layer includes all of the relevant first order logic rules for propositional connectives 
% (including the law of excluded middle). For the order relation it is axiomitized to be a linear relation. 

% We may additionally derive other connectives: 
% \begin{align*}
% 	\lnotcst{p} & \triangleq \limpcst{p}{\bot} \\
% 	T_1 \neq T_2 & \triangleq \lnotcst{\eqcst{T_1}{T_2}} \\
% 	T_1 < T_2 & \triangleq \landcst{\leqcst{T_1}{T_2}}{(T_1 \neq T_2)} \\
% 	T_1 \geq T_2 & \triangleq \leqcst{T_2}{T_1} \\
% 	T_1 > T_2 & \triangleq T_2 < T_1
% \end{align*}

% The full set of rules are listed as follows:

% %% Propositional rules
% \begin{mathpar}
% \inferrule
%   {\strut}
%   {\calG; \calF, p \entails{p}}
	
% \inferrule
%   {\strut}
%   {\calG; \calF \entails{\top}}

% \inferrule
%   {\calG; \calF \entails{\bot}}
%   {\calG; \calF \entails{p}}

% \inferrule
%   {\calG; \calF \entails{p_1} \\
%    \calG; \calF \entails{p_2}}
%   {\calG; \calF \entails{\landcst{p_1}{p_2}}}

% \inferrule
%   {\calG; \calF \entails{\landcst{p_1}{p_2}}}
%   {\calG; \calF \entails{p_1}}

% \inferrule
%   {\calG; \calF \entails{\landcst{p_1}{p_2}}}
%   {\calG; \calF \entails{p_2}}

% \inferrule
%   {\calG; \calF \entails{p_1}}
%   {\calG; \calF \entails{\lorcst{p_1}{p_2}}}

% \inferrule
%   {\calG; \calF \entails{p_2}}
%   {\calG; \calF \entails{\lorcst{p_1}{p_2}}}

% \inferrule
%   {\calG; \calF \entails{\landcst{p_1}{p_2}} \\
%    \calG; \calF, p_1 \entails{p} \\
%    \calG; \calF, p_2 \entails{p}}
%   {\calG; \calF \entails{p}}

% \inferrule
%   {\calG; \calF, p_1 \entails{p_2}}
%   {\calG; \calF \entails{\limpcst{p_1}{p_2}}}

% \inferrule
%   {\calG; \calF \entails{\limpcst{p_1}{p_2}} \\
%    \calG; \calF \entails{p_1}}
%   {\calG; \calF \entails{p_2}}

% \inferrule
%   {\strut}
%   {\calG; \calF \entails{\lorcst{p}{\lnot p}}}
% \end{mathpar}

% %% Equality - Refl / Trans / Sym
% \begin{mathpar}
% \inferrule
%   {\strut}
%   {\calG; \calF \entails{\eqcst{T}{T}}}

% \inferrule
%   {\calG; \calF \entails{\eqcst{T_1}{T_2}}}
%   {\calG; \calF \entails{\eqcst{T_2}{T_1}}}
  
% \inferrule
%   { \calG; \calF \entails{\eqcst{T_1}{T_2}} \\
%     \calG; \calF \entails{\eqcst{T_2}{T_3}} }
%   {\calG; \calF \entails{\eqcst{T_1}{T_3}}} \\

% \inferrule
%   {\strut}
%   {\calG; \calF \entails{\eqcst{D}{D}}}

% \inferrule
%   {\calG; \calF \entails{\eqcst{D_1}{D_2}}}
%   {\calG; \calF \entails{\eqcst{D_2}{D_1}}}
  
% \inferrule
%   { \calG; \calF \entails{\eqcst{D_1}{D_2}} \\
%     \calG; \calF \entails{\eqcst{D_2}{D_3}} }
%   {\calG; \calF \entails{\eqcst{D_1}{D_3}}}
% \end{mathpar}

% %% Equality - Congurence

% \begin{mathpar}
% \inferrule
%   {\calG; \calF \entails{\eqcst{T_1}{T_2}} \\
%    \calG; \calF \entails{\eqcst{D_1}{D_2}}}
%   {\calG; \calF \entails{\eqcst{\fshiftcst{T_1}{D_1}}{\fshiftcst{T_2}{D_2}}}}

% \inferrule
%   {\calG; \calF \entails{\eqcst{D_1}{D_1'}} \\
%    \calG; \calF \entails{\eqcst{D_2}{D_2'}}}
%   {\calG; \calF \entails{\eqcst{\dsumcst{D_1}{D_2}}{\dsumcst{D_1'}{D_2'}}}}

% \inferrule
%   {\calG; \calF \entails{\eqcst{T_1}{T_1'}} \\
%    \calG; \calF \entails{\eqcst{T_2}{T_2'}}}
%   {\calG; \calF \entails{\eqcst{\ddiffcst{T_1}{T_2}}{\ddiffcst{T_1'}{T_2'}}}}

% \inferrule
%   {\calG; \calF \entails{\eqcst{T_1}{T_1'}} \\
%    \calG; \calF \entails{\eqcst{T_2}{T_2'}} \\
%    \calG; \calF \entails{\leqcst{T_1}{T_2}}}
%   {\calG, t; \calF \entails{\leqcst{T_1'}{T_2'}}}
% \end{mathpar}

% %% Equality - Axiomtization 
% \begin{mathpar}
% \inferrule
%   {\strut}
%   {\calG; \calF \entails{\eqcst{\fshiftcst{T}{\dzerocst}}{T}}}

% \inferrule
%   {\strut}
%   {\calG; \calF \entails{\eqcst{\fshiftcst{T_1}{(\ddiffcst{T_2}{T_3})}}{\fshiftcst{T_2}{(\ddiffcst{T_1}{T_3})}}}}

% \inferrule
%   {\strut}
%   {\calG; \calF \entails{\eqcst{\dsumcst{(\ddiffcst{T_1}{T_2})}{D}}{\ddiffcst{(\fshiftcst{T_1}{D})}{T_2}}}}

% \inferrule
%   {\strut}
%   {\calG; \calF \entails{\eqcst{\fshiftcst{T}{(\dsumcst{D_1}{D_2})}}{\fshiftcst{(\fshiftcst{T}{D_1})}{D_2}}}}

% % \inferrule
% %   {\strut}
% %   {\calG; \calF \entails{\eqcst{\ddiffcst{(\fshiftcst{T}{D})}{T}}{D}}}

% \inferrule
%   {\strut}
%   {\calG; \calF \entails{\eqcst{\dsumcst{D_1}{D_2}}{\dsumcst{D_2}{D_1}}}}

% \inferrule
%   {\strut}
%   {\calG; \calF \entails{\eqcst{\dsumcst{D_1}{(\dsumcst{D_2}{D_3})}}{\dsumcst{(\dsumcst{D_1}{D_2})}{D_3}}}}
% \end{mathpar}

% %% Ordering
% \begin{mathpar}
% \inferrule
%   {\strut}
%   {\calG; \calF \entails{\leqcst{T}{T}}}

% \inferrule
%   {\calG; \calF \entails{\leqcst{T_1}{T_2}} \\ 
%    \calG; \calF \entails{\leqcst{T_2}{T_3}}}
%   {\calG; \calF \entails{\leqcst{T_1}{T_3}}}

% \inferrule
%   {\calG; \calF \entails{\leqcst{T_1}{T_2}} \\ 
%    \calG; \calF \entails{\leqcst{T_2}{T_1}}}
%   {\calG; \calF \entails{\eqcst{T_1}{T_2}}}

% \inferrule
%   {\strut}
%   {\calG; \calF \entails{\lorcst{(T_1 < T_2)}{\lorcst{(\eqcst{T_1}{T_2})}}{(T_1 > T_2)}}}

% \inferrule
%   {\strut}
%   {\calG; \calF \entails{(T + \dunitcst) > T}}
% \end{mathpar}

\begin{notation}
Let $p$ be a proposition with a free temporal variable $t$, written as $p(t)$ (i.e. $p$ is a \emph{predicate} over $t$). 
Define $p(T) \triangleq \Subst{T}{t}{p}$, i.e. the predicate ``applied'' to the specific element $T$.
\end{notation}

\begin{lemma}
If $\calG, t; \calF, p(t) \entails{q(t)}$ and $\calG; \calF \entails{p(T)}$, 
then $\calG; \calF \entails{q(T)}$.
\end{lemma}

\emph{Remark.} The structure of natural numbers is a model of the temporal logic.

\begin{corollary}
The logic is consistent.
\end{corollary}

==> defns/translation.tex <==
%% Define macros for translations

\DeclareDocumentCommand{\Interp}{m}{\left\lceil{#1}\right\rceil}
\DeclareDocumentCommand{\Trn}{m}{\left\llbracket{#1}\right\rrbracket}

\DeclareDocumentCommand{\Trndeco}{m m}{{\left\llbracket{#2}\right\rrbracket}^{#1}}

\DeclareDocumentCommand{\Trndag}{m}{\Trndeco{\dagger}{#1}}
\DeclareDocumentCommand{\Trnstar}{m}{\Trndeco{\star}{#1}}
\DeclareDocumentCommand{\Trnast}{m}{\Trndeco{*}{#1}}

\DeclareDocumentCommand{\Trnbar}{m}{\overline{\left\llbracket{#1}\right\rrbracket}}




==> fig/trj-example.tex <==
\begin{tikzpicture}
  \draw (-1.5,0) -- (1.5,0);
  \draw (0,-1.5) -- (0,1.5);
\end{tikzpicture}

==> fig/types-car-key.tex <==
\begin{center}
\begin{minipage}[t]{0.5\textwidth}
\begin{tabbing}
$\mathsf{Key}\phantom{sent}$ \=$::= \larrstycst{\unitstycst}{(\bsumstycst{\mathsf{Present}}{\mathsf{Absent}})}$\\
$\mathsf{Present}$ \>$::= \larrstycst{\mathsf{Auth}}{\unitstycst}$
\end{tabbing}
\end{minipage}
\hspace{4mm}
\begin{minipage}[t]{0.5\textwidth}
\begin{tabbing}
$\mathsf{Auth}\phantom{nt}$ \= $::= \tensorstycst{\mathsf{Challenge}}{\larrstycst{\mathsf{Response}}{\unitstycst}}$ \\
$\mathsf{Absent}$ \> $::= \unitstycst$
\end{tabbing}
\end{minipage}
\end{center}

\begin{center}
\begin{minipage}[t]{1\textwidth}
\begin{tabbing}
$\mathsf{Key}\phantom{sent}$ \=$::= \tplarrstycst{t_0}{\top}{\tpunitstycst{t}{t \leq t_0+100}}{(\tpsumstycst{t_1}{t_1 \leq t_0+10}{\mathsf{Present}}{\mathsf{Absent}})}$\\
$\mathsf{Present}$ \>$::= \tplarrstycst{t_2}{t_2 \leq t_1+10}{\mathsf{Auth}}{\tpunitstycst{t}{t \leq t_0+100}}$\\
$\mathsf{Absent}$ \> $::= \tpunitstycst{t}{t \leq t_0+100}$ \\
$\mathsf{Auth}$ \> $::= \tptensorstycst{t_3}{t_3 \leq t_2+10}{\mathsf{Challenge}}{\tplarrstycst{t_4}{t_4 \leq t_3+5}{\mathsf{Response}}{\tpunitstycst{t}{t \leq t_0+100}}}$
\end{tabbing}
\end{minipage}
\end{center}

\begin{align*}
\kw{Key}     &\triangleq \querystycst{\unittycst}{(\bsumstycst{\kw{Present}}{\kw{Absent}})} \\
\kw{Present} &\triangleq \larrstycst{\kw{Auth}}{\unitstycst} \\
\kw{Absent}  &\triangleq \unitstycst \\
\kw{Auth}    &\triangleq \bangstycst{\tau}{\querystycst{\tau}{\unitstycst}} \\
\\
\kw{AtEnd}(t) &\triangleq (\eqcst{t}{\fshiftcst{t_0}{100}}) \\
\\
\kw{Key}     &\triangleq \tpquerystycst{t}{\eqcst{t_1}{t_0}}{\unittycst}{(\tpsumstycst{t_2}{\fbetween{t_1}{t_2}{\fshiftcst{t_1}{10}}}{\kw{Present}}{\kw{Absent}})} \\
\kw{Present} &\triangleq \tplarrstycst{t_3}{\eqcst{t_2}{t_3}}{\kw{Auth}}{\tpunitstycst{t_3}{\kw{AtEnd}(t_3)}} \\
\kw{Absent}  &\triangleq \tpunitstycst{t_3}{\kw{AtEnd}(t_3)} \\
\kw{Auth}    &\triangleq \tpbangstycst{t_4}{\eqcst{t_4}{t_3}}{\tau}{
				\tpquerystycst{t_5}{\fbetween{t_4}{t_5}{\fshiftcst{t_4}{5}}}{\tau}{
					\tpunitstycst{t_6}{\eqcst{t_5}{t_6}}}} \\
\\
\end{align*}


==> pfpl-defns/pat.tex <==
\newcommand{\RuleSort}{\Sort{Rule}}
\newcommand{\RulesSort}{\Sort{Rules}}
\newcommand{\PatSort}{\Sort{Pat}}
\newcommand{\ConSort}{\Sort{Constr}}

\newcommand{\matchabt}[2]{\OpABT{\kw{match}}{#1;#2}}
\newcommand{\matchcst}[2]{\kwop{match}{#1}\,\cdbraces{#2}}

\newcommand{\rulessepcst}{\mathbin{\cdbar}}
\newcommand{\rulesabt}[2]{\OpABT{\OpInst{\kw{rules}}{#1}}{#2}}
\newcommand{\rulescst}[2]{#2}
\newcommand{\rulesseqabt}[2]{\rulesabt{#1}{\seq{#1}{#2}}}
\newcommand{\rulesseqcst}[2]{\rulescst{#1}{\seqsep{\rulessepcst}{#1}{#2}}}

\newcommand{\ruleabt}[4]{\OpABT{\OpInst{\kw{rule}}{#1}}{#2;\AbsABT{#3}{#4}}}
\newcommand{\rulecst}[4]{\pairff{#2}{#4}}

\newcommand{\rulenabt}[4]{\ruleabt{#1}{#2}{\seq{#1}{#3}}{#4}}
\newcommand{\rulencst}[4]{\rulecst{#1}{#2}{\seq{#1}{#3}}{#4}}
\newcommand{\rulepcst}[4]{\pairff{#2}{#4}}

\newcommand{\varexabt}[1]{\OpInst{\kw{var}}{#1}}
\newcommand{\varexcst}[1]{#1}

\newcommand{\holepatabt}{\circ}
%\newcommand{\holepatcst}{\circ}
\newcommand{\varpatabt}[1]{#1}
\newcommand{\varpatcst}[1]{#1}
\newcommand{\wildpatabt}{\kw{wild}}
\newcommand{\wildpatcst}{\kw{\_}}
\newcommand{\unitpatabt}{\unitexabt}
\newcommand{\unitpatcst}{\unitexcst}
\newcommand{\pairpatabt}[2]{\pairexabt{#1}{#2}}
\newcommand{\pairpatcst}[2]{\pairexcst{#1}{#2}}
\newcommand{\inpatabt}[2]{\OpABT{\OpInst{\kw{in}}{#1}}{#2}}
\newcommand{\inlpatabt}[1]{\inpatabt{\kw{l}}{#1}}
\newcommand{\inrpatabt}[1]{\inpatabt{\kw{r}}{#1}}
\newcommand{\inpatcst}[2]{{#1}\cdot{#2}}
\newcommand{\inlpatcst}[1]{\inpatcst{\kw{l}}{#1}}
\newcommand{\inrpatcst}[1]{\inpatcst{\kw{r}}{#1}}

\newcommand{\trpatcst}{\trexcst}
\newcommand{\fapatcst}{\faexcst}

\newcommand{\IsOfPat}[3]{{#3}\vdash\IsOf{#1}{#2}}
\newcommand{\IsOfExp}[3]{{#1}\vdash\IsOf{#2}{#3}}
\newcommand{\IsOfRule}[3]{\IsOf{#1}{#2}\mathbin{\rightsquigarrow}{#3}}
\newcommand{\IsOfRules}[3]{\IsOf{#1}{#2}\mathbin{\rightsquigarrow}{#3}}

\newcommand{\PatMatch}[3]{{#1}\vdash{#3}\mathrel{\triangleleft}{#2}}
\newcommand{\PatMismatch}[2]{{#1}\mathrel{\perp}{#2}}

\newcommand{\trconabt}[1]{\OpInst{\kw{truth}}{#1}}
\newcommand{\trconcst}[1]{\top}
\newcommand{\andconabt}[2]{\OpABT{\kw{and}}{#1;#2}}
\newcommand{\andconcst}[2]{{#1}\wedge{#2}}
\newcommand{\inlconabt}[3]{\inlexabt{#1}{#2}{#3}}
\newcommand{\inlconcst}[3]{\inlexcst{}{}{#3}}
\newcommand{\inrconabt}[3]{\inrexabt{#1}{#2}{#3}}
\newcommand{\inrconcst}[3]{\inrexcst{}{}{#3}}
\newcommand{\unitconabt}{\unitexabt}
\newcommand{\unitconcst}{\unitexcst}
\newcommand{\pairconabt}[2]{\pairexabt{#1}{#2}}
\newcommand{\pairconcst}[2]{\pairexcst{#1}{#2}}
\newcommand{\fstconabt}[1]{\fstexabt{#1}}
\newcommand{\fstconcst}[1]{\fstexcst{#1}}
\newcommand{\sndconabt}[1]{\sndexabt{#1}}
\newcommand{\sndconcst}[1]{\sndexcst{#1}}
\newcommand{\faconabt}[1]{\OpInst{\kw{falsity}}{#1}}
\newcommand{\faconcst}[1]{\perp}
\newcommand{\orconabt}[2]{\OpABT{\kw{or}}{#1;#2}}
\newcommand{\orconcst}[2]{{#1}\vee{#2}}

\newcommand{\sats}[2]{{#1}\models{#2}}
\newcommand{\negsats}[2]{{#1}\not\models{#2}}

%\newcommand{\entails}[2]{{#1}\leq{#2}}
%\newcommand{\negentails}[2]{{#1}\not\leq{#2}}

\newcommand{\contradictory}[1]{\JPost{#1}{\textsf{incon}}}

\newcommand{\IsOfPatC}[4]{{#3}\vdash\IsOf{#1}{#2}\;\sqbracks{#4}}
\newcommand{\IsOfRuleC}[4]{\IsOf{#1}{#2}\mathbin{\rightsquigarrow}{#3}\;\sqbracks{#4}}
\newcommand{\IsOfRulesC}[4]{\IsOf{#1}{#2}\mathbin{\rightsquigarrow}{#3}\;\sqbracks{#4}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "book"
%%% End: 


==> rules/lang-wfmd.tex <==
$\boxed{\calG; \calF \entails{\IsSType{A}}}$
\begin{mathpar}
\inferrule[]
{\calG, t; \calF \entails{\IsProp{p}}}
{\calG; \calF \entails{\IsSType{\tpunitstycst{t}{p}}}}

\inferrule[]
{\calG, t; \calF \entails{\IsProp{c}} \\  
 \calG, t; \calF \entails{\IsSType{A_1}} \\ 
 \calG, t; \calF \entails{\IsSType{A_2}} }
{\calG \entails{\IsSType{\tptensorstycst{t}{p}{A_1}{A_2}}}}

\inferrule[]
{\calG, t; \calF \entails{\IsProp{c}} \\  
 \calG, t; \calF \entails{\IsSType{A_1}} \\ 
 \calG, t; \calF \entails{\IsSType{A_2}} }
{\calG; \calF \entails{\IsSType{\tplarrstycst{t}{p}{A_1}{A_2}}}}

\inferrule[]
{\calG, t; \calF \entails{\IsProp{p}} \\  
 \calG, t; \calF \entails{\IsSType{A_1}} \\ 
 \calF, t; \calF \entails{\IsSType{A_2}} }
{\calG; \calF \entails{\IsSType{\tpsumstycst{t}{p}{A_1}{A_2}}}}

\inferrule[]
{\calG, t; \calF \entails{\IsProp{p}} \\  
 \calG, t; \calF \entails{\IsSType{A_1}} \\ 
 \calG, t; \calF \entails{\IsSType{A_2}} }
{\calG; \calF \entails{\IsSType{\tpwithstycst{t}{p}{A_1}{A_2}}}}
\end{mathpar}

$\boxed{\calG; \calF \entails{\IsCtx{\Delta}}}$
\begin{mathpar}
\inferrule
{\strut}
{\calG; \calF \entails{\IsCtx{\emptyset}}}

\inferrule
{\calG; \calF \entails{\IsCtx{\Delta}} \\ 
 \calG; \calF \entails{\IsSType{A}}}
{\calG; \calF \entails{\IsCtx{(\emptyset, \IsOf{x}{A})}}}
\end{mathpar}

==> rules/tlogic-truth.tex <==
$\boxed{\calG; \calF; \entails{p}}$

\vspace{1em}\textsc{Propositional}
\begin{mathpar}
\inferrule
  {\strut}
  {\calG; \calF, p \entails{p}}
	
\inferrule
  {\strut}
  {\calG; \calF \entails{\top}}

\inferrule
  {\calG; \calF \entails{\bot}}
  {\calG; \calF \entails{p}}

\inferrule
  {\calG; \calF \entails{p_1} \\
   \calG; \calF \entails{p_2}}
  {\calG; \calF \entails{\landcst{p_1}{p_2}}}

\inferrule
  {\calG; \calF \entails{\landcst{p_1}{p_2}}}
  {\calG; \calF \entails{p_1}}

\inferrule
  {\calG; \calF \entails{\landcst{p_1}{p_2}}}
  {\calG; \calF \entails{p_2}}

\inferrule
  {\calG; \calF \entails{p_1}}
  {\calG; \calF \entails{\lorcst{p_1}{p_2}}}

\inferrule
  {\calG; \calF \entails{p_2}}
  {\calG; \calF \entails{\lorcst{p_1}{p_2}}}

\inferrule
  {\calG; \calF \entails{\landcst{p_1}{p_2}} \\
   \calG; \calF, p_1 \entails{p} \\
   \calG; \calF, p_2 \entails{p}}
  {\calG; \calF \entails{p}}

\inferrule
  {\calG; \calF, p_1 \entails{p_2}}
  {\calG; \calF \entails{\limpcst{p_1}{p_2}}}

\inferrule
  {\calG; \calF \entails{\limpcst{p_1}{p_2}} \\
   \calG; \calF \entails{p_1}}
  {\calG; \calF \entails{p_2}}

\inferrule
  {\strut}
  {\calG; \calF \entails{\lorcst{p}{\lnot p}}}
\end{mathpar}

%% Equality - Refl / Trans / Sym
\noindent \textsc{Equality - Reflexivity, Transitivity, Symmetry}
\begin{mathpar}
\inferrule
  {\strut}
  {\calG; \calF \entails{\eqcst{T}{T}}}

\inferrule
  {\calG; \calF \entails{\eqcst{T_1}{T_2}}}
  {\calG; \calF \entails{\eqcst{T_2}{T_1}}}
  
\inferrule
  { \calG; \calF \entails{\eqcst{T_1}{T_2}} \\
    \calG; \calF \entails{\eqcst{T_2}{T_3}} }
  {\calG; \calF \entails{\eqcst{T_1}{T_3}}} \\

\inferrule
  {\strut}
  {\calG; \calF \entails{\eqcst{D}{D}}}

\inferrule
  {\calG; \calF \entails{\eqcst{D_1}{D_2}}}
  {\calG; \calF \entails{\eqcst{D_2}{D_1}}}
  
\inferrule
  { \calG; \calF \entails{\eqcst{D_1}{D_2}} \\
    \calG; \calF \entails{\eqcst{D_2}{D_3}} }
  {\calG; \calF \entails{\eqcst{D_1}{D_3}}}
\end{mathpar}

%% Equality - Congurence
\noindent \textsc{Equality - Congurence}

\begin{mathpar}
\inferrule
  {\calG; \calF \entails{\eqcst{T_1}{T_2}} \\
   \calG; \calF \entails{\eqcst{D_1}{D_2}}}
  {\calG; \calF \entails{\eqcst{\fshiftcst{T_1}{D_1}}{\fshiftcst{T_2}{D_2}}}}

\inferrule
  {\calG; \calF \entails{\eqcst{D_1}{D_1'}} \\
   \calG; \calF \entails{\eqcst{D_2}{D_2'}}}
  {\calG; \calF \entails{\eqcst{\dsumcst{D_1}{D_2}}{\dsumcst{D_1'}{D_2'}}}}

\inferrule
  {\calG; \calF \entails{\eqcst{T_1}{T_1'}} \\
   \calG; \calF \entails{\eqcst{T_2}{T_2'}}}
  {\calG; \calF \entails{\eqcst{\ddiffcst{T_1}{T_2}}{\ddiffcst{T_1'}{T_2'}}}}

\inferrule
  {\calG; \calF \entails{\eqcst{T_1}{T_1'}} \\
   \calG; \calF \entails{\eqcst{T_2}{T_2'}} \\
   \calG; \calF \entails{\leqcst{T_1}{T_2}}}
  {\calG, t; \calF \entails{\leqcst{T_1'}{T_2'}}}
\end{mathpar}

%% Equality - Axiomatization 
\noindent \textsc{Equality - Axiomatization}
\begin{mathpar}
\inferrule
  {\strut}
  {\calG; \calF \entails{\eqcst{\fshiftcst{T}{\dzerocst}}{T}}}

\inferrule
  {\strut}
  {\calG; \calF \entails{\eqcst{\fshiftcst{T_1}{(\ddiffcst{T_2}{T_3})}}{\fshiftcst{T_2}{(\ddiffcst{T_1}{T_3})}}}}

\inferrule
  {\strut}
  {\calG; \calF \entails{\eqcst{\dsumcst{(\ddiffcst{T_1}{T_2})}{D}}{\ddiffcst{(\fshiftcst{T_1}{D})}{T_2}}}}

\inferrule
  {\strut}
  {\calG; \calF \entails{\eqcst{\fshiftcst{T}{(\dsumcst{D_1}{D_2})}}{\fshiftcst{(\fshiftcst{T}{D_1})}{D_2}}}}

\inferrule
  {\strut}
  {\calG; \calF \entails{\eqcst{\dsumcst{D_1}{D_2}}{\dsumcst{D_2}{D_1}}}}

\inferrule
  {\strut}
  {\calG; \calF \entails{\eqcst{\dsumcst{D_1}{(\dsumcst{D_2}{D_3})}}{\dsumcst{(\dsumcst{D_1}{D_2})}{D_3}}}}
\end{mathpar}

%% Ordering
\noindent \textsc{Ordering}
\begin{mathpar}
\inferrule
  {\strut}
  {\calG; \calF \entails{\leqcst{T}{T}}}

\inferrule
  {\calG; \calF \entails{\leqcst{T_1}{T_2}} \\ 
   \calG; \calF \entails{\leqcst{T_2}{T_3}}}
  {\calG; \calF \entails{\leqcst{T_1}{T_3}}}

\inferrule
  {\calG; \calF \entails{\leqcst{T_1}{T_2}} \\ 
   \calG; \calF \entails{\leqcst{T_2}{T_1}}}
  {\calG; \calF \entails{\eqcst{T_1}{T_2}}}

\inferrule
  {\strut}
  {\calG; \calF \entails{\lorcst{(T_1 < T_2)}{\lorcst{(\eqcst{T_1}{T_2})}}{(T_1 > T_2)}}}

\inferrule
  {\strut}
  {\calG; \calF \entails{(T + \dunitcst) > T}}
\end{mathpar}

==> rules/tlogic-wfmd.tex <==
$\boxed{\calG; \calF \entails{\IsProp{p}}}$
\begin{mathpar}
\inferrule[]
{\strut}
{\calG; \calF \entails{\IsProp{\topcst}}}

\inferrule[]
{\strut}
{\calG; \calF \entails{\IsProp{\botcst}}}

\inferrule[]
{\calG; \calF \entails{\IsProp{p_1}} \\ 
 \calG; \calF \entails{\IsProp{p_2}}}
{\calG; \calF \entails{\IsProp{\landcst{p_1}{p_2}}}}

\inferrule[]
{\calG; \calF \entails{\IsProp{p_1}} \\ 
 \calG; \calF \entails{\IsProp{p_2}}}
{\calG; \calF \entails{\IsProp{\lorcst{p_1}{p_2}}}}

\inferrule[]
{\calG; \calF \entails{\IsProp{p_1}} \\ 
 \calG; \calF \entails{\IsProp{p_2}}}
{\calG; \calF \entails{\IsProp{\limpcst{p_1}{p_2}}}}

\inferrule[]
{\calG; \calF \entails{\IsTime{T_1}} \\
 \calG; \calF \entails{\IsTime{T_2}}}
{\calG; \calF \entails{\IsProp{\leqcst{T_1}{T_2}}}}

\inferrule[]
{\calG; \calF \entails{\IsTime{T_1}} \\ 
 \calG; \calF \entails{\IsTime{T_2}}}
{\calG; \calF \entails{\IsProp{\eqcst{T_1}{T_2}}}}

\inferrule[]
{\calG; \calF \entails{\IsDuration{D_1}} \\ 
 \calG; \calF \entails{\IsDuration{D_2}}}
{\calG; \calF \entails{\IsProp{\eqcst{D_1}{D_2}}}}
\end{mathpar}

$\boxed{\calG; \calF \entails{\IsTime{T}}}$
$\boxed{\calG; \calF \entails{\IsDuration{D}}}$
\begin{mathpar}
\inferrule
{\strut}
{\calG, t; \calF \entails{\IsTime{t}}}

\inferrule
{\strut}
{\calG; \calF \entails{\IsTime{\finitcst}}}

\inferrule
{\calG; \calF \entails{\IsTime{T}} \\
 \calG; \calF \entails{\IsDuration{D}}}
{\calG; \calF \entails{\IsTime{\fshiftcst{T}{D}}}}

\inferrule
{\strut}
{\calG; \calF \entails{\IsDuration{\dzerocst}}}

\inferrule
{\strut}
{\calG; \calF \entails{\IsDuration{\dunitcst}}}

\inferrule
{\calG; \calF \entails{\IsDuration{D_1}} \\
 \calG; \calF \entails{\IsDuration{D_2}}}
{\calG; \calF \entails{\IsDuration{\dsumcst{D_1}{D_2}}}}

\inferrule
{\calG; \calF \entails{\IsTime{T_1}} \\
 \calG; \calF \entails{\IsTime{T_2}}}
{\calG; \calF \entails{\IsDuration{\ddiffcst{T_1}{T_2}}}}
\end{mathpar}

$\boxed{\IsFCtx{\calG; \calF}}$
\begin{mathpar}
\inferrule
  {\strut}
  {\IsFCtx{\emptyset; \emptyset}}

\inferrule
  {\IsFCtx{(\calG; \calF)}}
  {\IsFCtx{(\calG, t; \calF)}}

\inferrule
  {\IsFCtx{(\calG; \calF)} \\ 
   \calG; \calF \entails{\IsProp{p}}}
  {\IsFCtx{(\calG; \calF, p)}}
\end{mathpar}


==> sections/abstract-old.tex <==
Communication protocols often come with temporal constraints that
restrict the \emph{timing} of interactions between processes.
This paper introduces \emph{temporal intuitionistic linear logic session types (\tilst)},
which augment intuitionistic linear logic session types with timing constraints,
facilitating the specification and verification of such protocols.
To show that well-typed processes never go wrong and are \emph{never late},
the paper contributes a \emph{semantic} logical relation and
proves the type system sound with respect to the logical relation.
The logical relation embodies the semantic \emph{asymmetry} arising from the passage of time and 
% The logical relation characterizes a process term by its progression through time
% using the notion of a \emph{computable trajectory}.
equips a process term with a \emph{computable trajectory} characterizing its progression through time. 
Trajectories are algebraic and vital to the temporal closure properties.
% between uses and provisions of temporal session types.

==> sections/conclusions.tex <==
This paper contributes temporal intuitionistic linear logic session types (\tilst),
a binary session type system facilitating the verification of protocols with temporal predicates.
To prove that well-typed \tilst programs meet their deadlines,
the paper develops the---to the best of our knowledge---first fully semantic logical relation for session-typed concurrency,
featuring computable trajectories and temporal closure.
%
\tilst and the logical relation are phrased for the terminating fragment of \ilst.
Support of recursive behavior, possibly by means of coinductive types,
amounts to an interesting future research endeavor.

%

% This paper brings flexible temporal predicates to the family of intuitionistic linear logic session types.
% We develop the theory of \tilst through the, to our knowledge, 
% first fully semantic logical relation for session-typed concurrency.
% %
% Handling computation and recursion requires extensions to our logical relation
% we consider non-trivial future work.
% %
% In many IoT and related applications, computations and looping are suitably constrained to be orthogonal to \tilst.
% For these, \tilst captures a powerful set of temporal properties,
% allows feasible typechecking, and can express real-world constraints.

==> sections/introduction-old.tex <==
% \begin{itemize}
% \item Example
% \item Brief sentences on models of time. (Constrast logical clocks from Dist-Sys)
% \end{itemize}

\emph{Session types} \cite{HondaCONCUR1993,HondaESOP1998,HondaPOPL2008} have emerged as a successful paradigm
for verifying programs consisting of concurrent, often distributed, processes that
use message passing to communicate. 
Session types capture \emph{protocols}, and allow specification of message content, sequencing, and branching.
This paper examines session types that constrain not only the sequencing of messages
but also their \emph{temporal dependencies}.

Specifically, it contributes \emph{temporal intuitionistic linear logic session types} (\tilst),
enriching communication protocols with temporal predicates.
\tilst is a descendant of the family of intuitionistic linear logic session types (\ilst)
\cite{CairesCONCUR2010,ToninhoESOP2013,CairesARTICLE2016},
which build on a Curry-Howard correspondence between the session-typed $\pi$-calculus and linear logic
\cite{CairesCONCUR2010,WadlerICFP2012}.
This strong logical foundation naturally instills \tilst with desirable properties,
such as deadlock freedom and protocol adherence.

The integration of time, logic, and computation has a rich history.
Various modal logics, such as linear temporal logics (LTL)~\cite{PnueliFOCS1977},
temporally relate the truth of propositions, formalizing notions such as \emph{always} 
and \emph{until} via modalities.
In these settings time itself is not the subject matter of the logic.
Logical studies into notions of time itself broadly divide into two categories:
\emph{interval-based models} and \emph{instant-based models} \cite{TemporalLogicSEP}.

Distributed systems applications consider \emph{logical clocks}~\cite{lamportclock},
which are partial orders between observable events.
In these settings time is implicit. No inference can be made about 
other parts of the system solely from the local progression of time. 
Time is abstract, local, and non-physical.
%
More related to our work are session types based on timed automata~\cite{BartolettiARTICLE2017,BocchiESOP2019},
which consider a synchronized, explicit and global notion of time. 
In these systems, communications specify a \emph{guard condition} in terms of actual 
passage of time tracked using local clocks.

\tilst instead adopts an instant-based model of time, treating points in time (namely, instants)
as the primary notion. Armed with a model of time, our system allows programs
to quantify over points in time at which a communication may occur. We attach
\emph{temporal predicates} to the usual session type connectives. This model 
matches the dynamic semantics of our system: communications are assumed to happen 
at an instant.

We adopt the method of \emph{logical relations}~\cite{TaitARTICLE1967,PlotkinTR1973,StatmanARTICLE1985,PittsStarkHOOTS1998} 
for \tilst, and define \emph{semantic inhabitance} of types purely based on execution behavior.
Freeing inhabitance from syntactic well-typedness allows for a constructive (\aka computational) standpoint, known as \emph{semantic typing}
\cite{LoefARTICLE1982,ConstableBook1986,TimanyUnpublished2022}.
Our logical relation enables us to study the semantics of programs whose temporal behavior is semantically significant, 
and to show that our \tilst programs actually adhere to the specified protocol. 
This entails strong properties such as deadlock freedom and termination.
Developing the logical relation highlights a few key changes to the proof method to accommodate 
temporal significance of program execution.

\begin{itemize}
  \item We identify computable trajectories as a crucial semantic device. We 
        further define necessary operations on computable trajectories and prove them to be well-behaving.
  \item We generalize forward and backwards closure properties of traditional logical relations 
  to account for progression of time. 
  \item The logical relation witnesses the inherent asymmetry between uses and provisions of sessions 
    induced by the passage of time. 
\end{itemize}


==> sections/key-ideas.tex <==
This section provides a high-level overview of our contributions.
Our aim is to distill the essence in broad strokes, hiding or possibly skipping over details.
Sections \cref{main:sec:key-ideas:types}, \cref{main:sec:key-ideas:implementation}, and \cref{main:sec:key-ideas:relation}
echo sections \cref{main:sec:tillst}, \cref{main:sec:implementation}, and \cref{main:sec:tslr}, \resp
which deliver a detailed presentation.

\subsection{Motivation}
\label{main:sec:key-ideas:motivation}

Correctness in many real-world communication protocols is defined not only by the adherence of all participants to the structure of
the protocol, but also by the timing of communications. Not adhering to timing constraints of a protocol can impact not only 
the correctness of computed values, but also the security requirements of applications.  

% \subsection{Prescribing Temporal Protocols with Temporal Session Types}
% \label{main:sec:key-ideas:types}

% Formally, temporal predicates are propositions $p$ under a binder $t$, written as $\AbsABT{t}{p}$.
% Notation $p(T)$ stands for $\Subst{T}{t}{p}$.
% When the predicate is attached to a type operator, the variable $t$ binds the time of the communication event for later reference. 
% For example, the receipt of the wake message by the car key has the associated predicate $t.\eqcst{t_1}{t_0}$,
% indicating that the key is willing to receive the wake message at a time $t_1$ that is precisely the protocol starting time $t_0$.
% The time $t_1$ is then used in the predicate $\fbetween{t_1}{t_2}{\fshiftcst{t_1}{10}}$ associated with the key's response, present or absent,
% indicating that the key will respond within $10$ units of time after the last interaction at $t_1$, the receipt of the wake message.

% Since protocols in \ilst are described from the point of view of the provider,
% it is also the provider that \emph{imposes} a temporal predicate.
% The client, on the other hand, must \emph{satisfy} the temporal predicate by \emph{instantiating} the time variable
% with a time for which the predicate holds.
% %
% These roles can easily be reversed using \emph{higher-order channels},
% \ie channels of type $\tplarrstycst{t}{p}{A_1}{A_2}$ and $\tptensorstycst{t}{p}{A_1}{A_2}$.

% Lastly we remark that \tilst allows consecutive communications to happen at the same time.
% % as witnessed by $\kw{Present}$ and $\kw{Auth}$ that demand the authentication channel and challenge message to arrive at the same time $t_2$.
% This choice is descriptive of our application domain,
% which requires communication events to be linearly ordered relative to an \emph{external} clock,
% shared among all communicating entities.
% Given the nondeterminism inherent to this domain,
% it is entirely conceivable that various communication events happen simultaneously.
% \ilst is phrased in terms of an \emph{instant-based} model of time \cite{TemporalLogicSEP},
% assuming a suitable notion of unit of time. 

% To conclude, we introduce temporal predicates in \tilst. This allow us to specify the timing of communication precisely. 
% There are previous works about timing constraints with communication. Timed session types \cite{BocchiESOP2019}
% has similar temporal constrains but each constraint depends on local clocks as comparing to \tilst with a global clock
% that all participants share a synchronous view of time. Rate-based session types \cite{IraciOOPSLA2023} proposes
% a periodic construct operates on a fixed time interval with a global clock. It, however, does not allow specifying 
% timing constraints on communication but rather on periodic constructs. As such, it would be difficult to encode a tightly 
% bounded communication we need such as the car key example.

\subsection{A Semantic Logical Relation for Temporal Protocol Adherence}
\label{main:sec:key-ideas:relation}

% With \tilst in hand, we can specify temporal constraints of embedded systems protocols.
% To verify that our \tilst programs actually adhere to the specified protocol
% we must typecheck the programs and additionally prove that typechecking is sufficient to establish soundness.
% For the latter, we carried out a mathematical proof that all well-typed \tilst programs are sound.
% Soundness here goes beyond typical type soundness and additionally entails the guarantee that processes do \emph{meet their deadlines}.

% These kinds of proofs are hard, or even impossible, to carry out using a standard progress-and-preservation argument
% \cite{HarperBOOK2016}.
% More suitable is the method of \emph{logical relations} \cite{TaitARTICLE1967,PlotkinTR1973,StatmanARTICLE1985,PittsStarkHOOTS1998}.
% As a proof method, logical relations allow us to enrich types with the property of interest,
% yielding stronger inductive hypotheses to conclude our proofs.
% As a semantic device, logical relations allow us to prescribe the properties that inhabitants of a type should have.
% The latter insight fueled a constructive (\aka computational) standpoint, typically referred to as \emph{semantic typing}
% \cite{LoefARTICLE1982,ConstableBook1986,TimanyJACM2024},
% making the definition of the logical relation independent of well-typedness.
% Such a semantic approach has the benefit that it can not only be used to show that well-typed programs have the property of interest,
% \yytodo{Reviewer A PLDI'24 complains about wording. I don't see a problem?}
% via the proof of the fundamental theorem of the logical relation,
% but also any program, even untyped ones.

% A contribution of this paper is the development of a \emph{semantic logical relation} for temporal protocol adherence.
% Although logical relations have been introduced for session-typed languages
% \cite{PerezESOP2012,CairesESOP2013,PerezARTICLE2014,DeYoungFSCD2020,DerakhshanLICS2021,BalzerARXIV2023},
% these prior logical relations are all dependent on well-typedness.
% In contrast, our \emph{temporal semantic session logical relation (\tslr)} is not reliant on well-typedness,
% and thus fully semantic.
% %
% Especially in our targeted application domain,
% semantic typing is advantageous because it facilitates integration with existing workflows for embedded system design.



==> sections/related.tex <==
% The Stanford Encyclopedia of Philosophy provides a nice introduction to \emph{Temporal Logic}
% (\url{https://plato.stanford.edu/entries/logic-temporal/}).

\sbtodo{Support of higher-order channels and spawning is another distinguishing feature of our work.
The former we use in our example.  We should work out which other works support those features as well.}

Our work most closely relates to
work that provides an intuitionistic, logic-based account of Metric Temporal Logic (MTL)
\cite{KoymansARTICLE1990,OuaknineWorrellLICS2005} as well as
work that augments session types with timing constraints.
%
The former is proof-theoretic,
whereas our work adopts \emph{semantic typing}
\cite{LoefARTICLE1982,ConstableBook1986,TimanyJACM2024}
based on \emph{logical relations} \cite{TaitARTICLE1967,PlotkinTR1973,StatmanARTICLE1985,PittsStarkHOOTS1998}.
%
The latter considers Honda-style session types,
both binary \cite{HondaCONCUR1993,HondaESOP1998} and multiparty \cite{HondaPOPL2008},
whereas our work builds on the Curry-Howard correspondence between session-typed processes and \emph{intuitionistic linear logic}
\cite{CairesCONCUR2010}.

% \subsection{Intuitionistic Metric Temporal Logic (IMTL)}

de~Sa \emph{et~al.}~\cite{SaPPDP2023} contribute Intuitionistic Metric Temporal Logic (IMTL),
an intuitionistic account of Metric Temporal Logic (MTL) \cite{KoymansARTICLE1990,OuaknineWorrellLICS2005},
which in turn extends linear temporal logic (LTL) \cite{PnueliFOCS1977} with temporal \emph{intervals}.
Rather than interpreting propositions over models, as is done in prior work on MTL,
the authors view temporal logic through the lens of the propositions-as-types paradigm,
focusing on how propositions are proved.
A similar endeavor has been undertaken prior by Kojima et al.~\cite{KojimaIgarashiARTICLE2011},
albeit for linear temporal logic (LTL) \cite{PnueliFOCS1977} and a reduced set of temporal modalities.
The technical contributions comprise a syntactic proof of cut elimination, entailing not only consistency of the logic,
but also temporal causality (``future events cannot affect the present'') and
temporal monotonicity (``a proof can never move backwards in time'').
% The authors provide a case study to demonstrate how IMTL can model well-timed digital circuits.
%
Similarly to our work,
the authors assume an \emph{instant-based} model of time.
% witnessed by the fact that cut reductions happen at the judgmental present time.
Our work, however, differs in various regards.
Most importantly, \tilst is a programming language,
whereas IMTL is a logic.
While cut reductions in IMTL can be viewed as giving rise to temporal computations,
only by defining an actual execution dynamics can we express the passage of time
and really infuse meaning to an instant-based model of time.
Our dynamics is also fundamental to our semantic typing approach,
culminating in our metatheoretic results based on a logical relation.
Technically, our work is also more general, permitting timing constraints other than intervals, and
adopts linear logic and session types, whereas IMTL is phrased for a propositional logic with temporal connectives,
admitting weakening and contraction.
From a philosophical perspective, IMTL seems concerned with restricting temporal computations internally,
whereas timeliness in \tilst is governed by an external clock.
As such, IMTL is also related to prior work on intuitionistic LTL\cite{DasICFP2018,DasLICS2018}, 
an orthogonal aspect we defer to future work.

% They have a delay rule, which allows an interval judgement to be interpreted at a future time.

% Our primary propositional notions are conjuctions, disjuctions, implications, and an general less-or-equal-to relation.

% To allow for a computational interpretation via cut reductions, the starting point of an interval has to coincide with the time of the judgment (present time).
% To advance time, temporal connectives are introduced.
% So, in our setting, communications advance time, however, in the authors' setting only temporal connectives advance time.

% The authors introduce temporal connectives, box and diamond, to support sub-intervals, which means that the logic amounts to an interval-based temporal logic.

% \sbtodo{DONE UP TO HERE.}

In the multiparty session types setting, 
Bocchi et al.~\cite{BocchiCONCUR2014} and Bartoletti et al.~\cite{BartolettiARTICLE2017}
consider temporal guards on communications.
These systems assume local clocks and a fixed view of durations as rational numbers.
Our system is defined with respect to a single global clock abstracted over a model of time.
Temporal predicates may reference the time of any prior event in the protocol.
% Neykova et al.~\cite{NeykovaARTICLE2017} contribute an extension of the Scribble
% protocol description language for runtime monitoring of protocol adherence.
% Adding runtime monitoring to \tilst promises to be useful
% in practice but orthogonal to our current focus.
Multiparty reactive sessions (MRS) \cite{CanoTR2019} take a global view of time as discretized instants.
This synchronous reactive programming model of time has found applications to embedded systems problems
via languages such as Esterel \cite{BerryGonthierARTICLE1992,BerryBook1999} and Lustre \cite{HalbwachsARTICLE1991}.
MRS connects logical instants to the external world via reaction to events.
This means that constraints cannot be directly specified using physical notions of time.
Le Brun et al.~\cite{LeBrunDardhaESOP2023} use the concept of timeouts to model message delivery failure,
but similarly leave correspondence between timeout and physical time intentionally unspecified.

Bocchi et al.~\cite{BocchiESOP2019} extend temporal guards to asynchronous binary session types.
This too gives access only to local views of time.
The choice of asynchrony also leads to a subtyping relation 
that is covariant on output and contravariant on input times.
In a synchronous system, the time both participants communicate must coincide.
Safely substituting types in our synchronous system requires
retyping relations which distinguish the client and provider roles.
For protocols that require authentication, the distinction of which side may be more permissive is critical to correctness.

Rate-based session types (RBST) \cite{IraciOOPSLA2023} augment
binary session types with periodicity, specifying the parts of a protocol that repeat at a fixed interval.
% This combines with the communication structure to define a rate, 
% which forms the basis for a compatibility relation and a rate-safety property.
Periodicity is only concerned with control flow, and not tied to communications.
This is insufficient to express narrower constraints on specific events such as responding to a message within a specific interval from a previous message.
\tilst moreover supports process spawning and higher-order channels,
while maintaining deadlock freedom (a property RBST lacks).

\yytodo{Cite works on session type logical relations}

% \subsection{$\pi$-calculus}
% \paragraph{Work by \cite{KobayashiARTICLE2002}}
% \subsection{Linear temporal calculi}
% \paragraph{Work by \cite{CavePOPL2014}}
% \sbtodo{Should we include the references to communicating timed automata that we had in the proposal?}


==> sections/tslr-cut-out.tex <==
\subsubsection{Overview}

In a syntactic logical relations~\cite{CRARY2007259} argument, the semantics of programs are tied to the 
\emph{canonical forms}, \ie values, they compute. For \tilst, we care not only about what canonical forms are computed, 
but also that they are computed in a timely manner as dictated by the temporal predicate in the types. Therefore, 
our development utilizes \emph{trajectories} as a semantic device for this purpose. 


Section \cref{main:sec:tsslr:traj} formalizes trajectories and operations on them. 
Trajectories (denoted by $r$, $s$) are functions from \emph{points in time} to configurations,
characterizing the program execution state at each point in time. The type $\wp{A}{t}{p}$ picks out 
a subset of the points $T$ in time according to the predicate $p$, at which the shape of the configuration 
$r(T)$ must take a canonical form according to connective.

We are especially interested in the subset of trajectories that can be realized by some sequence $\sigma$. 
Intuitively, $\sigma$ is a discrete but computable counterpart for the more convenient notion of 
trajectories. Towards this end we define a relation $\Rel{r}{\sigma}$ asserting $r$ is computed by the 
sequence $\sigma$. An element of the relation is termed a \emph{computable trajectory}, or just \emph{trajectory}
for short.

Section \cref{main:sec:tsslr:traj} defines three important operations on computable trajectories, each responding to 
a semantic necessity arising from the judgmental structure.
The operations are shown to respect the computability relation and shown to commute and cancel properly. 
\begin{itemize}
  \item An \emph{interleaving} operator $\il{r_1}{r_2}$ combines two computable trajectories into one describing the 
  execution of their concurrent composition. This is necessary for handling contexts $\Delta$.
  \item The \emph{partitioning} operators $\lpar{r_1}{T}$ and $\rpar{r_2}{T}$ access the before-$T$ and after-$T$ component 
  of the trajectory, \respb. This is especially useful for moving antecedents forward in time.
  \item Dually, the \emph{concatenation} operator $\concat{r_1}{r_2}$ pieces two trajectories of connected domains together.
  This is useful for moving succedents $A$ backward in time.
\end{itemize}

Section \cref{main:sec:tsslr:lr} contains the definition of the logical relation. We define two pairs of 
relations $\LAnyInt{\wp{A}{t}{p}}{T}$ and $\VAnyInt{\mathcal{A}}{T}$, each pair can be either starred or not. 
The pair $\LAnyInt{\wp{A}{t}{p}}{T}$ accesses shapes of configurations at times $T$ prescribed by the predicate $p$, and the relation of $\VAnyInt{\mathcal{A}}{T}$ certifies the resulting configuration 
against a ``type'' $\mathcal{A}$ now with a specific $T$ substituted in. This mirrors the expression and value 
interpretation commonly found in the literature.

\yytodo{references type system} We respond to the semantic asymmetry described in \cref{main:sec:tillst} by defining a starred relation 
$\LSInt{\wp{A}{t}{p}}{T}$ for interpreting antecedents and $\LInt{\wp{A}{t}{p}}{T}$ for succedents. This structure is mirrored in 
$\VAnyInt{\mathcal{A}}{T}$ due to the mutual recursive nature of the definitions. 
The relation $\LSInt{\wp{A}{t}{p}}{T}$ certifies the trajectories only for times in the future $T$ because these are 
the times reachable by clients. The relation $\LInt{\wp{A}{t}{p}}{T}$ \emph{requires} all $p$-satisfying $T$ 
to follow $T$ because it is what the types internalize. The sequent calculus root of \tilst enables this setup, 
as the system separates the uses and provisions of the connectives.

Trajectories certified for $\LSInt{\wp{A}{t}{p}}{T}$ can be moved freely into futures $T'$ 
because $\LSInt{\wp{A}{t}{p}}{T'}$ is a weakening of $\LSInt{\wp{A}{t}{p}}{T}$ by dropping requirements pertaining 
to times between $T$ and $T'$. Dually, $\LInt{\wp{A}{t}{p}}{T}$ can be moved freely backwards in time 
to pasts $T'$ as $\LInt{\wp{A}{t}{p}}{T'}$ requires no more than what was already present, knowing that all $p$-satisfying 
points in time are futures of $T$ and therefore futures of $T'$. The relevant lemma, \cref{main:lem:closure}, witnesses a 
pair of \emph{temporal closure} properties, akin to forward and backward closure properties 
of traditional logical relations.

\yytodo{type system forward reference} On the other hand, the moves between $\LInt{\wp{A}{t}{p}}{T}$ and $\LSInt{\wp{A}{t}{p}}{T}$ are certified by the retyping
lemma (\cref{main:lem:retyping}). In a sequent calculus their presence is isolated to the rules \ruleref{rule:fwd}
and \ruleref{rule:cut}. These rules are the only places where types switch between antecedents and succedents.


\sbtodo{Begin cut from trajectories.}
Although the operations defined in this subsection play a minor role in the statement
of the fundamental theorem of our logical relation (\Cref{main:thm:ftlr}), they are essential to its proof. The interleaving operator is necessary for 
treating the channel variable context. Because the rules move time forward going 
from conclusion to premise, partitioning and concatenation allow us to move semantic
objects from one point in time to another, as we will see in \cref{lem:sem-retyping}
in the next section. This movement in time connects the premises to the conclusion, 
which are judgments asserted at different times.
\sbtodo{End cut from trajectories.}







==> tables/illst-types.tex <==
\begin{table}[t]\label{main:tbl:illst-types}
\caption{Intuitionistic linear logic session types (\ilst).}
\small
\begin{tabular}{@{}rl@{}}
\toprule 
Type ($A$) & Description \\
\midrule
$\unitstycst$ & Signal closure  \\
$\bsumstycst{A_1}{A_2}$   & Offers one of services $A_1$ or $A_2$ \\
$\bwithstycst{A_1}{A_2}$  & Offers a selection of service between $A_1$ or $A_2$. \\
$\tensorstycst{A_1}{A_2}$ & Provide both $A_1$ and $A_2$ by sending a channel $A_1$ and then as $A_2$. \\
$\larrstycst{A_1}{A_2}$   & Accepts a service $A_1$ in order to provide $A_2$.  \\
\toprule
\end{tabular}
\end{table}

